Conformalized Reachable Sets for Obstacle Avoidance With Spheres

Safe motion planning algorithms are necessary for deploying autonomous robots in unstructured environments. Motion plans must be safe to ensure that the robot does not harm humans or damage any nearby objects. Generating these motion plans in real-time is also important to ensure that the robot can adapt to sudden changes in its environment. Many trajectory optimization methods introduce heuristics that balance safety and real-time performance, potentially increasing the risk of the robot colliding with its environment. This paper addresses this challenge by proposing Conformalized Reachable Sets for Obstacle Avoidance With Spheres (CROWS). CROWS is a novel real-time, receding-horizon trajectory planner that generates probalistically-safe motion plans. Offline, CROWS learns a novel neural network-based representation of a spherebased reachable set that overapproximates the swept volume of the robot's motion. CROWS then uses conformal prediction to compute a confidence bound that provides a probabilistic safety guarantee on the learned reachable set. At runtime, CROWS performs trajectory optimization to select a trajectory that is probabilstically-guaranteed to be collision-free. We demonstrate that CROWS outperforms a variety of state-of-the-art methods in solving challenging motion planning tasks in cluttered environments while remaining collision-free. Code, data, and video demonstrations can be found at https://roahmlab.github.io/crows/

==> algorithms/online_planning.tex <==
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]
    \State {\bf Require:} $\tplan > 0$, $\Nt, N_s \in \N, \obsset, \SDF$, and $\texttt{cost}: K \to \R$.
    \State {\bf Initialize:} $i = 0$, $t_i = 0$, and \newline
    \phantom{\bf stupid} $\{ k^*_j \} = \texttt{Opt}(\qstart,\zeros,\zeros,\obsset,\texttt{cost}, \tplan, \Nt, N_s, \SDF, \sfo)$
    \State {\bf If} $k^*_{j} = \texttt{NaN}$, {\bf then} break
    \State{\bf Loop:}
    
        \State \hspace{0.05in} // Line \ref{lin:apply} executes simultaneously with Lines \ref{lin:opt} -- \ref{lin:else} //
        \State \hspace{0.05in}  // Use Lem. \ref{lem:sjo}, Thm. \ref{thm:sfo}, and Alg. \ref{alg:sdf}//  
        
        \hspace{0.05in} {\bf Execute} $q_d(t;k^*_i)$  on robot for $t \in [t_i,t_i + \tplan]$ \label{lin:apply} 
      \State \hspace{0.05in}  $\{ k^*_{i+1} \} = \texttt{Opt}(q_d(\tplan;k^*_j), \dot{q}^{j}_d(\tplan;k^*_j), \ddot{q}^{j}_d(\tplan;k^*_j),\obsset,$ \phantom{stupid stupid stupid}$\texttt{cost},\tplan, \Nt, N_s, \SDF, \sfo)$ \label{lin:opt} %Alg. \ref{alg:opt} \label{lin:opt}
        \State \hspace{0.05in} {\bf If} $k^*_{i+1} = \texttt{NaN}$, {\bf then} break
        \State \hspace{0.05in} {\bf Else}  $t_{i+1} \leftarrow t_i + \tplan$ and $i \leftarrow i + 1$ \label{lin:else}

    \State{\bf End}
    \State {\bf Execute} $q_d(t;k^*_i)$  on robot for $t \in [t_i+\tplan,t_i + \tfin]$ \label{lin:brake}
\end{algorithmic}
\caption{\small \methodname{} Online Planning}
\label{alg:online_planning}
\end{algorithm}

==> algorithms/pzfk.tex <==
%~~~~~~~~~~~~ Compose FK
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]

% \State{\bf parfor} $i = 1:\nt$ %// parallel for each time step

\State $\pz{p_0}(\pzqi) \leftarrow \zeros$ %// initialize frame location 

\State$ \pz{R_0}(\pzqi) \leftarrow I_{3 \times 3}$ %// initialize frame orientation


\State\hspace{0in}{\bf for} $j = 1:\nq$ %// for each joint

    % \State\hspace{0.2in}$\pz{R_{j}^{j-1}}(\pzqji), \pz{\nom{p\jssmu}} \leftarrow \texttt{pzTransMat}(\pzi{q_j})$ 
    
    \State\hspace{0.2in}$\pz{R_{j}^{j-1}}(\pzqji), \pz{p_j}(\pzqi) \leftarrow \pz{\homtrans_{j}^{j-1}}(\pzqji)$ %as in \eqref{eq:homogeneous_transform}
    
    \State\hspace{0.2in}$\pz{p_j}(\pzqi) \leftarrow \pz{p_{j-1}}(\pzqi) \oplus \pz{R_{j-1}}(\pzqi) \pz{p_{j}^{j-1}}$
        
    \State\hspace{0.2in}$ \pz{R_j}(\pzqi) \leftarrow  \pz{R_{j-1}}(\pzqi)  \pz{R_{j}^{j-1}}(\pzqji)$ 
    
    \State\hspace{0.2in}$\pz{\FK_j}(\pzqi) \leftarrow \{ \pz{R_j}(\pzqi) ,  \pz{p_j}(\pzqi) \}$ 
    
\State\hspace{0in}{\bf end for}

% \State{\bf end parfor}

\end{algorithmic}
\caption{\small $\{\pz{\FK_j}(\pzqi)\,:\, j \in \Nq \} = \texttt{PZFK}(\pzqi)$}
\label{alg:compose_fk}
\end{algorithm}

==> algorithms/pzsfo.tex <==
%~~~~~~~~~~~~ Compose SFO
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]

\State $\pz{p_0}(\pzqi) \leftarrow \zeros$ %// initialize frame location 

\State$ \pz{R_0}(\pzqi) \leftarrow I_{3 \times 3}$ %// initialize frame orientation


\State\hspace{0in}{\bf for} $j = 1:\nq$ %// for each joint

    \State\hspace{0.2in}$\pz{R_{j}^{j-1}}(\pzqji), \pz{\nom{p\jssmu}} \leftarrow \pz{\homtrans_{j}^{j-1}}(\pzqji)$ as in \eqref{eq:homogeneous_transform}
    
    \State\hspace{0.2in}$\pz{p_j}(\pzqi) \leftarrow \pz{p_{j-1}}(\pzqi) \oplus \pz{R_{j-1}}(\pzqi) \pz{p_{j}^{j-1}}$
        
    \State\hspace{0.2in}$ \pz{R_j}(\pzqi) \leftarrow  \pz{R_{j-1}}(\pzqi)  \pz{R_{j}^{j-1}}(\pzqji)$ 
    
    \State\hspace{0.2in}$\pz{\FK_j}(\pzqi) \leftarrow \{ \pz{R_j}(\pzqi) ,  \pz{p_j}(\pzqi) \}$ 
    
\State\hspace{0in}{\bf end for}

\end{algorithmic}
\caption{\small $\{\pz{\FK_j}(\pzqi)\,:\, j \in \Nq \} = \texttt{PZFK}(\pzqi)$}
\label{alg:compose_sfo}
\end{algorithm}

==> algorithms/rdf_alg.tex <==
\begin{algorithm}[t]
\begin{algorithmic}[1]
\State $\{\pzqi\,:\, i \in \Nt\} \leftarrow (q_0,\dot q_0)$ 
\State $\co, \Go \leftarrow O$ 
\State{\bf for} $i = 1:n_t$ %// for each time steps
    \State\hspace{0.2in}{\bf for} $j = 1:n_q$ % for each joint
        \State\hspace{0.4in} $\pzFOjKi \leftarrow \texttt{PZFO}(\pzqi)$ 
        \State\hspace{0.4in} $\pzFOjki \leftarrow \texttt{slice}(\pzFOjKi, k)$ \label{lst:line:fo}
        \State\hspace{0.4in} $\pzFOjkibuf \leftarrow \pzFOjki\oplus Z_O^g$ \label{lst:line:buffered_fo}
    \State\hspace{0.2in}{\bf end for}
\State{\bf end for}
\State{\bf for} $j = 1:n_q$
    \State\hspace{0.2in} $\Pj \leftarrow \conv(\bigcup_{i = 1}^{\nt}\pzFOjkibuf)$ \label{lst:line:conv}
    %\State\hspace{0.2in} $\{(A_j^{(h)},b_j^{(h)})\,:\, h \in \Nhj\} \leftarrow \texttt{polytope}(\mathcal{P}_j)$
    \State\hspace{0.2in} {\bf if} $c_O \in \Pj$ {\bf then}
    % \State\hspace{0.2in} {\bf if} $A_j\,c_O-b_j \leq 0$ {\bf then} // $c_0 \in \mathcal{P}_j$
        %\State\hspace{0.4in} $\Tilde{r}_j \leftarrow \max_{h\in\Nhj}\frac{A_j^{(h)}\,p-b_j^{(h)}}{||A_j^{(h)}||}$ // negative distance 
        \State\hspace{0.4in} $\ardf_j \leftarrow -\dist(\co,\partial\Pj)$ // negative distance 
    \State\hspace{0.2in} {\bf else}
        %\State\hspace{0.4in} $\Tilde{r}_j \leftarrow \texttt{QP}\left(c_O, \{(A_j^{(h)},b_j^{(h)})\,:\, h \in \Nhj\}\right)$ // positive distance
        \State\hspace{0.4in} $\ardf_j \leftarrow \dist(\co,\partial\Pj)$ // positive distance 
    \State\hspace{0.2in} {\bf end if} 
\State{\bf end for}
\State \textbf{Return} $\{\ardf_j\,:\, j \in \Nq\}$
\end{algorithmic}
\caption{\texttt{RDF}$(q_0, \dot q_0, k, O)$}
\label{alg:rdf}
\end{algorithm}

==> algorithms/sdf_algorithm.tex <==
\begin{algorithm}[t]
\begin{algorithmic}[1]
\State $A, b, E \leftarrow \mathcal{O}$
\State $d_{\text{face}} \leftarrow \max(Ac-b)$  %shortest distances between $c$ and $A$ 
\State{\bf if} $d_{\text{face}} \leq 0$ // check negative distances to faces
% \State{\bf if} $\max(Ac-b) \leq 0$
% \State\hspace{0.2in} \textbf{Return} $\max(Ac-b)$ // negative distance
\State\hspace{0.2in} \textbf{Return} $d_{\text{face}}$ 

\State{\bf else} // check positive distances to faces
% \State \hspace{0.2in} Compute $\text{proj}_{A} = c - (Ac-b) * A$ // perpendicular distance between $c$ and each face of $A$ 
% \State \hspace{0.2in} $C^{\perp} = \mathbf{1}_{m_A \times 1} \cdot c^{T} - \texttt{diag}(Ac-b) \cdot A$ \jon%// project $c$ onto each face $A$ 
\State\hspace{0.2in}{\bf for} $i_A = 1:m_A$ %// for each projection
    \State\hspace{0.4in} $d_{\text{face}} \leftarrow (A c- b)_{i_A}$
    % \State\hspace{0.4in} $p_{\text{face}} \leftarrow c - d_{\text{face}} \cdot A_{i_A}^{T}$
    % \State\hspace{0.4in} $d'_{\text{face}} \leftarrow \max(Ap_{\text{face}}-b)$
    % \State\hspace{0.4in} $p_{\text{face}} \leftarrow \max(A(c - d_{\text{face}} \cdot A_{i_A}^{T}) - b)$ 
    % \State\hspace{0.4in}{\bf if} $d_{\text{face}} \geq 0$ \textbf{and} $ p_{\text{face}} \leq 0$ 
    \State\hspace{0.4in} $p_{\text{face}} \leftarrow c - d_{\text{face}} \cdot A_{i_A}^{T} $ 
    \State\hspace{0.4in}{\bf if} $d_{\text{face}} \geq 0$ \textbf{and} $ \max(A p_{\text{face}} - b) \leq 0$ 
        \State\hspace{0.6in} \textbf{Return} $d_{\text{face}}$
    \State\hspace{0.4in}{\bf end if}
    \State\hspace{0.2in}{\bf end for}
\State{\bf end if}
\State $d_{\text{edge}} \leftarrow \inf$
\State{\bf for} $i_E = 1: |E|$ // check distances to edges%for every edge e in E, we compute the distance from c to e, and take the minimum
\State\hspace{0.2in} $d_{\text{edge}} \leftarrow \min(\dist(c,E_{i_E}), d_{\text{edge}})$
\State{\bf end for}
\State \textbf{Return} $d_{\text{edge}}$
\end{algorithmic}
\caption{\SDF$(\mathcal{O}, c)$ }
\label{alg:sdf}
\end{algorithm}


==> algorithms/vertex_enumeration.tex <==
\begin{algorithm}[t]
    \caption{Zonotope Vertex Enumeration}
    \label{alg:vertex_enumeration}
    \begin{algorithmic}[1]
        \REQUIRE Zonotope $Z \subset \mathbb{R}^2$ with $n \in \mathbb{N}$ generators $g_1, \cdots, g_n$ \jon{should 1 and 2 be under required?}
        \STATE \quad Multiply any generator with negative y-value by $-1$.
        \STATE \quad Reduce generators $g_1, \cdots, g_n$ to $g\prime_1, \cdots, g\prime_m$ by\\
        \quad  summing generators with the same direction $(m \leq n)$.
        \STATE \quad Sort $g\prime_1, \cdots, g\prime_m$ by angle in ascending order. 
        \STATE \quad Compute vertex coefficient matrix $C \in \mathbb{R}^{m \times m}$ such that
        \begin{equation*}
            C(i,j) = 
            \begin{cases}
                1 & \text{if } j \geq i \\
                -1 & \text{otherwise}
            \end{cases}.
        \end{equation*}
        \STATE \quad  Compute the $2m$ vertices $\{v_1, \cdots, v_{2m}\}$:
        \begin{align*}
            v_k &= c + \sum_{j=1}^{m} C(k,j) g_j \\
            v_{m+k} &= c - \sum_{j=1}^{m} C(k,j) g_j. 
       \end{align*}
        \STATE \textbf{End}
    \end{algorithmic}
\end{algorithm}

==> sections/03_modeling.tex <==
\section{Arm and Environment Modeling}
\label{sec:modeling}
This section summarizes the environment, obstacles, and robot models used throughout the remainder of the paper. 

\subsection{Environment}\label{subsec:env}
The arm must avoid obstacles in the environment while performing safe motion planning. 
We begin by stating an assumption about the environment and its obstacles:
\begin{assum} \label{assum:env}
The robot and obstacles are all located in a fixed inertial world reference frame, which we denote $W \subset \R^{3}$.
We assume the origin of $\world$ is known and that each obstacle is represented relative to the origin of $\world$.
At any time, the number of obstacles $\nObs \in \N$ in the world is finite.
Let $\obsset = \{ O_1, O_2, \ldots, O_{\nObs} \}$ be the set of all obstacles.
Each obstacle is convex, bounded, and static with respect to time.
For each obstacle, we have access to a zonotope that overapproximates the obstacle's volume. See Fig. \ref{fig:assumption_figure}.
\end{assum}

\noindent Note that any convex, bounded object can always be overapproximated by a zonotope \cite{guibas2003zonotopes}.
In addition, any non-convex bounded obstacle can be outerapproximated by its convex hull.
For the remainder of this document, safety is checked using the zonotope overapproximation of each obstacle.

% conflate every obstacle with its zonotope overapproximation because we use the zonotope representation during safe motion planning \Ram{when we check safety do we do it with the zonotope overapproximation or with the original obstacle? Maybe want to clarify that point here.}.


\subsection{Arm Kinematics}\label{subsec:arm}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\columnwidth]{figures/spharmour_modeling.pdf}
    \caption{A visualization of the robot arm and its environment.
    The obstacles are shown in red and the robot is shown in grey (translucent).
    The volume of each joint is overapproximated by a sphere, shown in purple, in the workspace.
    Each link volume is overapproximated by a tapered capsule formed by the convex hull shown in light purple of two consecutive joint spheres (Assum. \ref{assum:joint_link_occupancy}).}
    \label{fig:assumption_figure}
    \vspace*{-0.3cm}
\end{figure}
This work considers an $\nq$ degree of freedom serial robotic manipulator with configuration space $Q$.
Given a compact time interval $T \subset \R$, we define a trajectory for the configuration as $q: T \to Q \subset \R^{\nq}$ and a trajectory for the velocity as $\dot{q}: T \to \R^{\nq}$.
% Let $\Nq = \{1,\ldots,\nq\}$.
We make the following assumptions about the structure of the robot model:

\begin{assum}\label{assum:robot}
The robot operates in a three dimensional workspace, denoted $\workspace \subset \R^{3}$, such that $\workspace \subset \world$.
There exists a reference frame called the base frame, which we denote the $0$\ts{th} frame, that indicates the origin of the robot's kinematic chain.
The transformation between the robot's base frame and the origin of the world frame is known.
The robot is fully actuated and composed of only revolute joints, where the $j$\ts{th} joint actuates the robot's $j$\ts{th} link.
The robot's $j$\ts{th} joint has position and velocity limits given by $\qj \in [\qlim^-, \qlim^+]$ and $\qdj \in [\dqlim^-, \dqlim^+]$ for all $t \in T$, respectively. 
The robot's input is given by $u: T \to \R^{\nq}$.
\end{assum}

Recall from Assum. \ref{assum:robot} that the transformation from \textit{world} from to the the robot's $0$\ts{th}, or \textit{base}, frame is known.
We further assume that the $j$\ts{th} reference frame $\{\hat{x}_j, \hat{y}_j, \hat{z}_j\}$ is attached to the robot's $j$\ts{th} revolute joint, and that $\hat{z}_j = [0, 0, 1]^\top$ corresponds to the $j$\ts{th} joint's axis of rotation.
% Then for a time-dependent configuration, $\q$, the position and orientation of frame $j$ with respect to frame $j-1$ can be expressed as a homogeneous transformation matrix \cite[Ch. 2]{spong2005textbook}: \jon{Feel like we can drop this \eqref{eq:homogeneous_transform}}
% \begin{equation} \label{eq:homogeneous_transform}
%     \homtrans_{j}^{j-1}(\qj) = 
%     \begin{bmatrix} R\jssmu (\qj) & p\jssmu \\
%     \zeros  & 1 \\
%     \end{bmatrix},
% \end{equation}
% where $R\jssmu (\qj)$ is a configuration-dependent rotation matrix and $p\jssmu$ is the fixed translation vector from frame $j-1$ to frame $j$.

% We can now use \eqref{eq:homogeneous_transform} to express the forward kinematics of the robot.
% Let $\FK_j: Q \to \R^{4 \times 4}$ map the robot's configuration to the pose of the $j$\ts{th} joint in the world frame:
Then the forward kinematics $\FK_j: Q \to \R^{4 \times 4}$ maps a time-dependent configuration, $\q$, to the pose of the $j$\ts{th} joint in the world frame:
\begin{equation}\label{eq:fk_j}
    \FK_j(\q) = 
    \prod_{l=1}^{j} \homtrans_{l}^{l-1}(q_l(t)) = 
    \begin{bmatrix} R_j(\q) & p_j(\q) \\
    \zeros  & 1 \\
    \end{bmatrix},
\end{equation}
where 
\begin{equation}
    R_j(\q) \coloneqq R_j^{0}(\q) = \prod_{l=1}^{j}R_{l}^{l-1}(\ql)
\end{equation}
and 
\begin{equation}
    p_j(\q) = \sum_{l=1}^{j} R_{l}(\q) p_{l}^{l-1}.
\end{equation}

\noindent Note that we use the revolute joint portion of Assum. \ref{assum:robot} to simplify the description of forward kinematics; however, these assumptions and the methods described in the following sections can be readily be extended to other joint types such as prismatic or spherical joints in a straightforward fashion.
Note that the lack of input constraints means that one could apply an inverse dynamics controller \cite{Caccavale2020} to track any trajectory of the robot perfectly.
It is also possible to deal with the tracking error due to uncertainty in the robot's dynamics \cite{michaux2023armour}.
However, this is outside of the scope of the current work and as a result, we focus exclusively on modeling the kinematic behavior of the manipulator.


\subsection{Arm Occupancy}\label{subsec:arm_occupancy}
Next, we use the arm's kinematics to define the \textit{forward occupancy} which is the volume occupied by the arm in the workspace.
Let $L_j \subset \R^3$ denote the volume occupied by the $j$\ts{th} link with respect to the $j$\ts{th} reference frame. 
Then the forward occupancy of link $j$ is the map $\FO_j: Q \to \pow{\workspace}$ defined as
\begin{align}\label{eq:link_occupancy}
     \FO_j(\q) &= p_j(\q) \oplus R_j(\q) L_j,
\end{align}
where $p_j(\q)$ the position of joint $j$ and $R_j(\q) L_j$ is the rotated volume of link $j$.
The volume occupied by the entire arm in the workspace is given by the function $\FO: Q \to \workspace$ that is defined as
\begin{align}\label{eq:forward_occupancy}
    \FO(\q) = \bigcup_{j = 1}^{\nq} \FO_j(\q) \subset \workspace. 
\end{align}

Note that any of the robot's link volumes $L_j$ may be arbitrarily complex.
We therefore introduce an assumption to simplify the construction of the reachable set in Sec. \ref{subsec:sfo_construction}:
\begin{assum}\label{assum:joint_link_occupancy}
    For every $j \in \{1,\dots, \nq\}$ there exists a sphere of radius $r_j$ with center $p_j(\q)$ that overapproximates the volume occupied by the $j$\ts{th} joint in $\workspace$.
    Furthermore, the link volume $L_j$ is a subset of the tapered capsule formed by the convex hull of the spheres overapproximating the $j$\ts{th} and $j+1$\ts{th} joints.
    See Fig. \ref{fig:assumption_figure}.
\end{assum}
Following Assum. \ref{assum:joint_link_occupancy}, we define the sphere $\Sjq$ overapproximating the $j$\ts{th} joint as 
\begin{equation}\label{eq:joint_occupancy}
    \Sjq = B(p_j(\q), r_j)
\end{equation}
and the tapered capsule $TC_j(q(t))$ overapproximating the $j$\ts{th} link as
\begin{equation}
 TC_j(q(t)) = \conv\Big( \Sjq \cup \Sjpq \Big).
\end{equation}
Then, \eqref{eq:link_occupancy} and \eqref{eq:forward_occupancy} can then be overapproximated by
\begin{align}\label{eq:link_capsule_occupancy}
     \FO_j(\q)  &\subset \conv\Big( \Sjq \cup \Sjpq \Big) \nonumber \\
     &= TC_j(q(t)),
\end{align}
and
\begin{equation} \label{eq:forward_capsule_occupancy}
    \FO(\q) \subset \bigcup_{j = 1}^{\nq} TC_j(q(t)) \subset \workspace, 
\end{equation}
respectively.

% \begin{enumerate}
%     \item \Ram{probably need to explain that this assumption is easy to satisfy and then explain why.}
% \end{enumerate}

For convenience, we use the notation $\FO(q(T))$ to denote the forward occupancy over an entire time interval $T$.
Note that we say that the arm is \textit{in collision} with an obstacle if $\FO_j(\q) \cap O_{\ell} \neq \emptyset$ for any $j \in \Nq$ or $\ell \in \NObs$ where $\NObs = \{1,\ldots,\nObs\}$.
 

\input{algorithms/pzfk}
\subsection{Trajectory Design}\label{subsec:trajectory_design}
\methodname{} computes safe trajectories  by solving an optimization program over parameterized trajectories at each planning iteration in a receding-horizon manner.
Offline, we pre-specify a continuum of trajectories over a compact set $K \subset \R^{n_k}$, $n_k \in \N$. 
Then each trajectory, defined over a compact time interval $T$, is uniquely determined by a \textit{trajectory parameter} $k \in K$.
Note that we design $K$ for safe manipulator motion planning, but $K$ may also be designed for other robot morphologies or to accommodate additional tasks \cite{holmes2020armtd, kousik2020bridging, kousik2019safe, liu2022refine} as long as it satisfies the following properties:
\begin{defn}[Trajectory Parameters]
\label{defn:traj_param}
For each $k \in K$, a \emph{parameterized trajectory} is an analytic function $q(\,\cdot\,; k) : T \to Q$ that satisfies the following properties:
\begin{outline}[enumerate]
\1 The parameterized trajectory starts at a specified initial condition $(q_0, \dot{q}_0)$, so that $q(0; k) = q_0$, and $\dot{q}(0; k) = \dot{q}_0$.
\1 Each parameterized trajectory brakes to a stop such that $\dot{q}(\tfin; k) = 0$.
\end{outline}
\end{defn}
\noindent \methodname{} performs real-time receding horizon planning by executing the desired trajectory computed at the previous planning iteration while constructing the next desired trajectory for the subsequent time interval.
Therefore, the first property ensures each parameterized trajectory is generated online and begins from the appropriate future initial condition of the robot.
The second property ensures that a braking maneuver is always available to bring the robot safely to a stop.

% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{figures/sfo_link_construction.pdf}
%     \caption{ 
%     A visualization of the \SFO construction for a robotic arm in 3D.
%     (First column) The planning time horizon is partitioned into a finite set of polynomial zonotopes (Sec. \ref{subsubsec:pz_time_horizon}) before computing the parameterized trajectory polynomial zonotopes shown in purple (Sec. \ref{subsubsec:pz_desired_traj}).
%     The time horizon consists of a planning phase $[0,\tplan)$ and a braking phase $[\tplan, \tfin]$.
%     A single desired trajectory for each joint is shown in black.
%     (Second column) The polynomial zonotope forward kinematics algorithm (Sec. \ref{subsubsec:pzfk}) computes an overapproximation of the joint positions for each time interval.
%     (Third column) The joint position zonotopes are first overapproximated by axis-aligned boxes and (Fourth column) subsequently overapproximated by the smallest sphere that circumscribes the box (Sec. \ref{subsubsec:sjo}).
%     For the sake of clarity, the insets in columns 2 through 4 depict the polynomial zonotope joint positions, overapproximating boxes, and the circumscribed spheres as larger.
%     (Fifth column) The radii of the circumscribed spheres are then added to the radii of the nominal joint spheres (Assum. \ref{assum:joint_link_occupancy}) to produce the \SJO (Lem. \ref{lem:sjo}).
%     (Sixth column) Finally, the \SFO is computed for each link corresponding to the desired trajectory.
%     (Seventh column) Note that \methodname generates link occupancies that are less conservative than previous reachability methods \cite{holmes2020armtd, michaux2023armour}.
%     }\label{fig:sfo_3D}
% \end{figure*}
%~~~~~~~~~~~~~~~~~~~ OLD TEXT
% \subsection{Obstacles}
% The arm must avoid obstacles in the environment while performing motion planning. 
% These obstacles satisfy the following assumption:
% % We denote the set of obstacles as a set $O \subset W$.
% % We make the following assumptions about obstacles:
% \begin{assum}
% \label{assum:obstacles}
% The transformation between the world frame of the workspace and the base frame of the robot is known, and obstacles are represented in the base frame of the robot.
% At any time, the number of obstacles $\nObs \in \N$ in the scene is finite.
% Let $\obsset$ be the set of all obstacles $\{ O_1, O_2, \ldots, O_{\nObs} \}$.
% Each obstacle is convex, bounded, and static with respect to time.
% The arm has access to a zonotope that overapproximates the obstacle's volume in workspace.
% Each zonotope overapproximation of the obstacle has the same volume and is an axis-aligned cube.
% % \yong{In our case, we assumed all the obstacles are the same size of axis-aligned cubes.}
% \end{assum}

% If one has an obstacle that is larger than the pre-fixed axis-aligned cube, then one can introduce several axis-aligned cubes whose union is an overapproximation to the obstacle. 


% Dynamic obstacles may also be considered within the \methodname framework by introducing a more general notion of safety \cite[Definition 11]{vaskov2019towards}, but we omit this case in this paper to ease exposition.
% Finally, if a portion of the scene is occluded then one can treat that portion of the scene as an 




% \begin{equation} \label{eq:forward_capsule_occupancy}
%     \FO(\q) \subset \bigcup_{j = 1}^{\nq} \conv\Big( B(p_j(\q), r_j) \cup B(p_{j+1}(\q), r_{j+1})\Big) \subset \workspace, 
% \end{equation}

==> sections/04_spherical_forward_occupancy.tex <==
\section{Planning Algorithm Formulation}\label{sec:planning}
% The goal of this work is to construct a collision free trajectory in a receding-horizon fashion.
% One could accomplish this by solving the following nonlinear optimization problem at each planning iteration:
The goal of this work is to construct collision free trajectories in a receding-horizon fashion by solving the following nonlinear optimization problem at each planning iteration:
\begin{align}
    \label{eq:optcost}
    &\underset{k\in K}{\min} &&\texttt{cost}(k) \\
    \label{eq:optpos}
    &&& q_j(t; k) \in [\qlim^-, \qlim^+]  &\forall t \in T, j \in \Nq \\
    \label{eq:optvel}
    &&& \dot{q}_j(t; k) \in [\dqlim^-, \dqlim^+]  &\forall t \in T,   j \in \Nq \\
    \label{eq:optcolcon}
    &&& \FO_j(q(t; k)) \bigcap \obsset = \emptyset  &\forall t \in T,   j \in \Nq
\end{align}
The cost function \eqref{eq:optcost} specifies a user- or task-defined objective, while each constraint guarantees the safety of any feasible parameterized trajectory.
The first two constraints ensure that the trajectory does not violate the robot's joint position \eqref{eq:optpos} and velocity limits \eqref{eq:optvel}.
The last constraint \eqref{eq:optcolcon} ensures that the robot does not collide with any obstacles in the environment.

Implementing a real-time algorithm to solve this optimization problem is challenging for two reasons.
First, obstacle-avoidance constraints are typically non-convex \cite{borrelli2020collision}. 
Second, each constraint must be satisfied for all time $t$ in a continuous, and uncountable, time interval $T$.
To address these challenges, this section develops \methodname a novel, real-time trajectory planning method that combines reachability analysis with differentiable collision primitives. 
We first discuss how to overapproximate a family of parameterized trajectories that the robot follows.
Next, we discuss how to overapproximate \eqref{eq:forward_capsule_occupancy} using the Spherical Forward Occupancy ($\sfo$).
Then, we discuss how to compute the signed distances between the forward occupancy and obstacles in the robot's environment.
Finally, in Sec. \ref{subsec:online_planning} we discuss how to combine the $\sfo$ and signed distance function to generate obstacle-avoidance constraints for a real-time algorithm that can be used for safe online motion planning.


\subsection{Polynomial Zonotope Trajectories and Forward Kinematics}\label{subsec:pz_traj}
This subsection summarizes the relevant results from \cite{michaux2023armour} that are used to overapproximate parameterized trajectories (Def. \ref{defn:traj_param}) using polynomial zonotopes.

\subsubsection{Time Horizon and Trajectory Parameter PZs}\label{subsubsec:pz_time_horizon}
We first describe how to create polynomial zonotopes representing the planning time horizon $T$.
We choose a timestep $\timestep$ so that $\nt \coloneqq \frac{T}{\timestep} \in \N$ divides the compact time horizon $T \subset \R$ into $\nt$ time subintervals denoted by $N_t := \{1,\ldots,\nt\}$.
We then represent the $i$\ts{th} time subinterval, corresponding to $t \in \iv{(i-1)\timestep, i\timestep}$, as a polynomial zonotope $\pz{T_i}$, where 
\begin{equation}
    \label{eq:time_pz}
    \pz{T_i} =
        \left\{t \in T \mid 
            t = \tfrac{(i-1) + i}{2}\timestep + \tfrac{1}{2} \timestep \tvari,\ \tvari \in [-1,1]
        \right\}
\end{equation}
with indeterminate $\tvari \in \iv{-1, 1}$.
We also use polynomial zonotopes to represent the set of trajectory parameters $K$.
For each $j \in \{1, \dots, \nq\}$, $\Kj$ is the compact one-dimensional interval  $\Kj = \iv{-1, 1}$ such that $K$ is given by the Cartesian product $K = \bigtimes_{i=1}^{n_q} K_i$.
Following \eqref{eq:int_to_pz}, we represent the interval $\Kj$ as a polynomial zonotope $\pz{\Kj} = \kjvar$ where $\kjvar \in \iv{-1, 1}$ is an indeterminate.


\subsubsection{Parameterized Trajectories}\label{subsubsec:pz_desired_traj}
Using the time partition $\pz{T_i}$ and trajectory parameter $\pz{K_j}$ polynomial zonotopes described above, we create polynomial zonotopes $\pzqji$ and $\pzqdji$ that overapproximate the parameterized position (Fig. \ref{fig:sfo_3D}, col. 1) and velocity trajectories defined in Def. \ref{defn:traj_param} for all $t$ in the $i$\ts{th} time subinterval. 
This is accomplished by plugging $\pz{T_i}$ and $\pz{K}$ into the formulas for $\qkj$ and $\qdkj$.
For convenience, we restate \cite[Lemma 14]{michaux2023armour} which proves that sliced position and velocity polynomial zonotopes are overapproximative:
\begin{lem}[Parameterized Trajectory PZs]
\label{lem:pz_desired_trajectory}
The parameterized trajectory polynomial zonotopes $\pzqji$ are overapproximative, i.e., for each $j \in \Nq$ and $k\in \pz{K_j},$ 
\begin{equation}
    \qkj \in \pzqjki \quad \forall t \in \pz{T_i}
\end{equation}
One can similarly define $\pzqdji$ that are also overapproximative. 
\end{lem}

\subsubsection{PZ Forward Kinematics}\label{subsubsec:pzfk}
We begin by representing the robot's forward kinematics \eqref{eq:fk_j} using polynomial zonotope overapproximations of the joint position trajectories.
Using $\pzqi$, we compute $\pz{p_j}(\pzqi)$ and $\pz{R_j}(\pzqi)$, which represent overapproximations of the position and orientation of the $j$\ts{th} frame with respect to frame $(j-1)$ at the $i$\ts{th} time step.
% Because all operations involving polynomial zonotopes are either exact or overapproximative, 
The polynomial zonotope forward kinematics can be computed (Alg. \ref{alg:compose_fk}) in a similar fashion to the classical formulation \eqref{eq:fk_j}.
For convenience, we restate \cite[Lemma 17]{michaux2023armour} that proves that this is overapproximative:
\begin{lem}[PZ Forward Kinematics]
\label{lem:PZFK}
Let the polynomial zonotope forward kinematics for the $j$\ts{th} frame at the $i$\ts{th} time step be defined as
\begin{equation}\label{eq:pzfk_j}
    \pzFKjKi = 
    \begin{bmatrix} \pz{R_j}(\pzqi) & \pz{p_j}(\pzqi)\\
    \mathbf{0}  & 1 \\
    \end{bmatrix},
\end{equation}
where
\begin{align}
    \pz{R_j}(\pzqi) &= \prod_{l=1}^{j} \pz{R_{l}^{l-1}}(\pzqli), \\
    \pz{p_j}(\pzqi) &= \sum_{l=1}^{j} \pz{R_l}(\pzqi) \pz{p_{l}^{l-1}},
\end{align}
then for each  $j \in \Nq$,  $k \in \pz{K}$,  $\FK_j(q(t;k)) \in  \pzFKjki$ for all $t \in \pz{T_i}$.
\end{lem}


\subsection{\SFO Construction}\label{subsec:sfo_construction}
This subsection describes how to use the parameterized trajectory polynomial zonotopes discussed in Section \ref{subsec:pz_traj} to construct the \SFO{} introduced in Section \ref{subsubsec:sfo}.
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ SPHERICAL JOINT OCCUPANCY
\subsubsection{\SJO}\label{subsubsec:sjo}
We next introduce the \SJO to compute an overapproximation of the spherical volume occupied by each arm joint in the workspace.
In particular, we show how to construct a sphere that overapproximates the volume occupied by the $j$\ts{th} joint over the $i$\ts{th} time interval $\pz{T_i}$ given a parameterized trajectory polynomial zonotope $\pzqi$.
First, we use the polynomial zonotope forward kinematics to compute $\pz{p_j}(\pzqi)$, which overapproximates the position of the $j$\ts{th} joint frame (Fig. \ref{fig:sfo_3D} col. 2).
Next, we decompose $\pz{p_j}(\pzqi)$ into
\begin{equation}
    \pz{p_j}(\pzqi) = \pzCjiK \oplus \pzuj,
\end{equation}
where $\pzCjiK$ is a polynomial zonotope that only contains generators that are dependent on $\pz{K}$, and $\pzuj$ is a zonotope that is independent of $\pz{K}$.
We then bound $\pzuj$ with an axis-aligned cube (Fig. \ref{fig:sfo_3D}, col. 3) that is subsequently bounded by a sphere (Fig. \ref{fig:sfo_3D}, col. 4) of radius $u_{j,i}$.
Finally, the \SJO is defined as
\begin{equation}
    \SjiK = \pzCjiK \oplus B(\mathbf{0}, r_j + u_{j,i}),
\end{equation}
where $\pzCjiK$ is a polynomial zonotope representation of the sphere center, $r_j$ is the radius nominal joint sphere, and $u_{j,i}$ is the sphere radius that represents additional uncertainty in the position of the joint.
Because $\pzCjiK$ is only dependent on $\pz{K}$, slicing a particular trajectory parameter $k \in K$ yields a single point for the sphere center $\pzCjik$. 
We state this result in the following lemma whose proof is in Appendix \ref{appendix:sjo}:

\begin{lem}[Spherical Joint Occupancy]\label{lem:sjo}
Let the \emph{Spherical Joint Occupancy} for the 
% Let $\pz{p_j}(\pzqi)$ be a polynomial zonotope overapprozimation for the position of the 
$j$\ts{th}  frame at the $i$\ts{th} time step be defined as
\begin{equation}
    \SjiK =\pzCjiK \oplus B(\mathbf{0}, r_j + u_{j,i}),
\end{equation}
where $\pzCjiK$ is the center of $\pz{p_j}(\pzqi)$, $r_{j}$ is the radius of $\Sjqk$, and $u_{j,i}$ is the radius of a sphere that bounds the independent generators of $\pz{p_j}(\pzqi)$.
Then,
\begin{equation}
    \Sjqk) \subset \Sjik
\end{equation}
for each  $j \in \Nq$,  $k \in \pz{K}$,  $\Sjqk \in  \Sjik$ for all $t \in \pz{T_i}$.
\end{lem}


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ SPHERICAL LINK OCCUPANCY
\subsubsection{\SFO}\label{subsubsec:sfo}

Previous work \cite{michaux2023armour} used \eqref{eq:link_occupancy} along with Lem. \ref{lem:PZFK} to overapproximate the forward occupancy of the $j$\ts{th} link over the $i$\ts{th} time step using polynomial zonotopes:
\begin{align}\label{eq:pz_forward_occupancy_j}
     \pzFOjKi = \pz{p_j}(\pzqi) \oplus \pz{R_j}(\pzqi)\pz{L_j}.
\end{align}

Our key insight is replacing \eqref{eq:link_occupancy} with an alternate representation based on a tapered capsule \eqref{eq:link_capsule_occupancy}.
Recall from Assum. \ref{assum:joint_link_occupancy} that the $j$\ts{th} link can be outer-approximated by the tapered capsule formed by the two spheres encompassing the closest joints.
Sec. \ref{subsubsec:sjo} described how to overapproximate each joint volume over a continuous time interval $\pz{T_i}$.
Therefore, by Assum. \ref{assum:joint_link_occupancy}, the volume occupied by $j$\ts{th} link over the $\pz{T_i}$ is overapproximated by the tapered capsule formed by $\Sjik$ and $\Sjpik$ for a given trajectory parameter $k \in K$:
\begin{equation}
    \TCjik = \conv(\Sjik \cup \Sjpik) \quad \forall t \in \pz{T_i}.
\end{equation}

However, tapered capsules are not ideal for performing collision checking with arbitrary, zonotope-based obstacles.
Instead, we introduce the \SFO ($\sfo$) to overapproximate $\TCjik$ with $\ns \in \N$ spheres (Fig. \ref{fig:sfo_3D}, col. 6):

\begin{thm}[Spherical Forward Occupancy]\label{thm:sfo}
Let $\ns \in \N$ be given and let the \emph{\SFO} for the $j$\ts{th} link at the $i$\ts{th} time step be defined as
\begin{equation}\label{eq:tapered_capsule_overapprox}
    % \sfojk = \left\{\Sbarjimk \, : \, 1 \leq m \leq \ns \right\},
    \sfojk = \left\{\Sbarjimk \, : \, m \in N_s \right\},
\end{equation}
where $N_s = \{1, \cdots, \ns\}$ and
\begin{equation}
    \Sbarjimk = B\left(\bar{c}_{j,i,m}(k), \bar{r}_{j,i,m}(k)\right),
\end{equation}
is the $m$\ts{th} link sphere with with center $\bar{c}_{j,i,m}(k)$ and radius $\bar{r}_{j,i,m}(k)$.
Then
\begin{equation}
    \TCjik \subset \sfojk
\end{equation}
for each  $j \in \Nq$,  $k \in \pz{K}$, and $t \in \pz{T_i}$.
\end{thm}
Theorem \ref{thm:sfo} yields a tighter reachable set (Fig. \ref{fig:sfo_3D}, col. 6) compared to previous methods (Fig. \ref{fig:sfo_3D}, col. 7) while remaining overapproximative. 
Sec. \ref{subsec:online_planning} describes how the \SFO is used to compute collision-avoidance constraints.

\input{algorithms/sdf_algorithm}


% \subsection{Exact Signed Distance Computation}\label{subsec:sdf}
% The Spherical Forward Occupancy constructed in \ref{subsubsec:sfo} is composed entirely of spheres, where each sphere can be considered a point with a margin of safety corresponding to its radius.
% Therefore, utilizing spheres within obstacle-avoidance constraints requires only point-to-obstacle distance calculations.
% To make use of this sphere-based representation for trajectory planning, this subsection presents Alg. \ref{alg:sdf} for computing the exact signed distance between a point and a zonotope in 3D based on the following lemma whose proof can be found in the appendix:
% \begin{lem}\label{lem:sdf}
% Given an obstacle zonotope $\mathcal{O} \in \R^3$, consider its polytope representation with normalized rows $(A,b)$ and edges $E$ computed from its vertex representation.
% Then for any point $c \in \R^3$,
% % \begin{equation}
% %     \sdf(c; \mathcal{O}) = 
% %         \begin{cases}
% %           \max(Ac-b)  & \text{if } c \in \mathcal{O} \\
% %           (Ac-b)_{i_A} & \text{if } c \not \in \mathcal{O}, \text{ but } \proj(c; A_{i_A}) \in \mathcal{O} \\
% %           \underset{E_{i_E} \in E}{\min} \dist(c; E_{i_E})  & \text{otherwise}
% %         \end{cases}    ,
% % \end{equation}
% \begin{equation}
%     \sdf(c; \mathcal{O}) = 
%         \begin{cases}
%           \max(Ac-b)  & \text{if } c \in \mathcal{O} \\
%           % (Ac-b)_{i_A} & \text{if } c \not \in \mathcal{O} \text{ and } \max(A p_{\text{face}} - b) \leq 0 \\
%           (Ac-b)_{i_A} & \text{if } c \not \in \mathcal{O}, \max(A p_{\text{face}} - b) \leq 0 \\
%           \underset{E_{i_E} \in E}{\min} \dist(c; E_{i_E})  & \text{otherwise}
%         \end{cases}    ,
% \end{equation}
% $i_A$ indexes the rows of $(Ac-b)$, $i_E$ indexes the edges of $E$, and $p_{\text{face}} = c - (Ac-b)_{i_A} \cdot A_{i_A}^{T}$ is the projection of $c$ onto the $i_A$\ts{th} hyperplane of $\mathcal{O}$ whose normal vector is given by $A_{i_A}^{T}$.
% \end{lem}

\subsection{Trajectory Optimization}\label{subsec:trajectory_optimization}
We combine parameterized polynomial zonotope trajectories (Sec. \ref{subsec:pz_traj}) with the \SFO (Sec. \ref{subsubsec:sfo}) and an exact signed distance function (Sec. \ref{subsec:sdf}) to formulate the following trajectory optimization problem:
\begin{align}
    \label{eq:pzoptcost}
    &\underset{k \in K}{\min} &&\numop{cost}(k) \hspace{3cm} \opt&  \\
    \label{eq:pz_optpos}
    &&& \hspace*{-0.75cm} \pzqjki \subseteq [\qlim^-, \qlim^+]  \hspace{1cm} \forall (i,j) \in N_t \times N_q \\
    \label{eq:pz_optvel}
    &&& \hspace*{-0.75cm}\pzqdjki \subseteq [\dqlim^-, \dqlim^+]  \hspace{1cm} \forall (i,j) \in N_t \times N_q \\
    \label{eq:pz_optcolcon}
    % &&& \hspace*{-0.75cm}\texttt{SDF}(\mathcal{O}_{n}, \bar{c}_{j,i,m}(k)) > \bar{r}_{j,i,m}(k) &\forall (i,j,m,n) \in N_t \times N_q \times N_s \times N_{\mathcal{O}},
    &&& \hspace*{-0.75cm}\texttt{SDF}(\mathcal{O}_{n}, \bar{c}_{j,i,m}(k)) > \bar{r}_{j,i,m}(k) \nonumber\\
    &&& \hspace{2.2cm} \forall (i,j,m,n) \in N_t \times N_q \times N_s \times N_{\mathcal{O}},
\end{align}
where $i \in N_t$ indexes the time intervals $\pz{T_i}$, $j \in N_q$ indexes the $j$\ts{th} robot joint, $m \in N_s$ indexes the spheres in each link forward occupancy, and $n \in N_{\mathcal{O}}$ indexes the number of obstacles in the environment.

\subsection{Safe Motion Planning}\label{subsec:online_planning}
\methodname's planning algorithm is summarized in Alg. \ref{alg:online_planning}.
The polytope representation $(A,b)$ and edges $E$ for computing the signed distance (Alg. \ref{alg:sdf}) to each obstacle $\mathcal{O}_n \in \obsset$ are computed offline before planning.
Every planning iteration is given $\tplan$ seconds to find a safe trajectory.
The $\sjo$ (Lem. \ref{lem:sjo}) is computed at the start of every planning iteration outside of the optimization problem and the $\sfo$ (Thm. \ref{thm:sfo}) is computed repeatedly while numerically solving the optimization problem. If a solution to \optref{} is not found, the output of Alg. \ref{alg:online_planning} is set to \nan and the robot executes a braking maneuver (Line \ref{lin:brake}) using the trajectory parameter found in the previous planning iteration.
To facilitate real-time motion planning, analytical constraint gradients for \eqref{eq:pz_optpos}--\eqref{eq:pz_optcolcon} are provided to aid computing the numerical solution of \optref.

\input{algorithms/online_planning}


% During optimization, the center polynomial zonotope is sliced to produce the expected center point, with the respective radii providing the uncertainty volume.
% During optimization, the jacobian is provided by the slice operation of the center polynomial zonotope as the radius does not change no matter how a specific time interval is sliced.

% Note in particular, that the construction and solving of the optimization problem described in lines \eqref{eq:pz_optpos}--\eqref{eq:pz_optcolcon} is given $t\plan$ time. 
% If a solution is not found within that time, then the output of Alg. \ref{alg:online_planning} is set to $\texttt{NaN}$.
% To facilitate real-time motion planning, we include the analytical constraint gradients when numerically solving \optref.
% As described above, each constraint contains a polynomial zonotope whose coefficients correspond to the trajectory parameters and are also the decision variables of the optimization problem.
% Because each polynomial zonotope can be viewed as a polynomial function solely of the trajectory parameters, we can compute each constraint gradient with respect to the trajectory parameter $k$ using the standard rules of differential calculus, \emph{i.e.}, the power, product, and chain rules.
 
% online planning constraints: \\
% Requires SJO, k, obsverts, obsedges \\
% create nn with obsverts, obsedges \\
% for each time and joint pair \\
% slice center pz \\
% solve for c \\
% solve for r \\
% dists <- query nn with c \\
% dists <- subtract r \\
% end for \\
% return -dists \\
% end \\
% \\
% sjo generation: \\
% requires q, q\_dot \\
% traj\_q <- q, q\_dot \\
% for each time and joint
% fk <- pzfk \\
% p, buf <- split\_pz(fk) \\
% r\_buf <- norm(to\_interval(buf)) \\
% r <- joint\_r + r\_buf \\
% end for \\
% return (p, r) \\

% \subsection{Theoretical Motion Planning Problem}



% \subsection{Offline Reachability Analysis}
% \label{sec:offline_reachability}

% \subsection{Offline Reachability Analysis}
% \label{sec:offline_reachability}


% \subsection{Online Optimization}
% \label{sec:online_optimization}

% \begin{align}
%     \label{eq:optcost}
%     &\underset{k\in K}{\min} &&\texttt{cost}(k) \\
%     \label{eq:optpos}
%     &&& q_j(t; k) \in [\qlim^-, \qlim^+]  &\forall t \in T, j \in \Nq \\
%     \label{eq:optvel}
%     &&& \dot{q}_j(t; k) \in [\dqlim^-, \dqlim^+]  &\forall t \in T,   j \in \Nq \\
%     \label{eq:optcolcon}
%     &&& \FO_j(q(t; k)) \bigcap \obsset = \emptyset  &\forall t \in T,   j \in \Nq
% \end{align}





% \begin{align*}
%     \label{eq:rdf-nn-optcost}
%     &\underset{k \in K}{\min} &&\texttt{cost}(k) \texttt{(Batched Opt)}  \\
%     &&&  \pzqjki \subseteq [\qlim^-, \qlim^+]  &\forall j\in\Nq,i\in \Nt\\
%     &&& \pzqdjki \subseteq [\dqlim^-, \dqlim^+]  &\forall j\in\Nq,t\in \Nt \\
%     &&& \label{eq:rdf-nn-col-avoid}
%     \texttt{SDF}(A_{\ell}, b_{\ell}, E_{\ell}, c_{j,i}) - r > 0   &\forall \ell\in\NObs \\
%     &&&
%     \texttt{SDF}(A_{\ell}, b_{\ell}, E_{\ell}, \bar{c}_{j,i,m}(k)) - \bar{r}_{j,i,m}(k) > 0  &\forall \ell\in\NObs 
% \end{align*}
% \subsubsection{Forward Occupancy Reachable Set}
% To ensure that the robot never collides with any obstacles, we overapproximate the forward occupancy \eqref{eq:forward_occupancy_j} of each link over every time interval.
% By applying the polynomial zonotope forward kinematics set and the fact that all operations involving polynomial zonotopes are either exact or overapproximative, the polynomial zonotope forward occupancy reachable set can be computed and proven to be overapproximative: 
% \begin{lem}[PZ Forward Occupancy]
% \label{lem:pz_fo}
% Let the $j$\ts{th} link of the robot be overapproximated by a polynomial zonotope denoted by $\pz{L_j}$ and the polynomial zonotope forward occupancy reachable set for the $j$\ts{th} link at the $i$\ts{th} time step be defined as:
% \begin{align}\label{eq:pz_forward_occupancy_j}
%      \pzFOjKi = \pz{p_j}(\pzqi) \oplus \pz{R_j}(\pzqi)\pz{L_j},
% \end{align}
% then for each $j \in \Nq$,  $k \in \pz{K}$, $\FO_j(q(t;k)) \in  \pzFOjki$ for all $t \in \pz{T_i}$.
% \end{lem}
% \noindent Sec. \ref{subsec:constraint_generation} describes how the forward occupancy reachable set is used to compute collision-avoidance constraints.
% % The Polynomial Zonotope Forward Occupancy Algorithm (PZFO), detailed in Alg. \ref{alg:compose_fo}, is identical to the PZFK algorithm but is applied to the volume of each link rather than joint positions.
% Let
% \begin{equation}
%     \label{eq:pz_forward_occupancy}
%     \pz{FO}(\pzqi) = \bigcup_{j = 1}^{\nq} \pzFOjKi.
% \end{equation}
% % \input{algorithms/pzfo}



% OLD INTRO STUFF
% how to construct the \SLO ($\slo$) to overoverapproximate the volume of each link of the robot during a trajectory.

% In this section we describe how to overapproximate the forward occupancy of the robot using spheres using reachability analysis.
% Finally, we discuss how the Spherical Forward Occupancy ($\sfo$ ) is constructed from the  $\sjo$ and $\slo$.
% Note in this optimization problem, we have assumed that the robot does not have to deal with self-intersection constraints. 

% This section develops a novel, differentiable reachable set representation for robot manipulators called the \SFO ($\sfo$).
% Similar to previous reachability-based planning methods \cite{holmes2020armtd, michaux2023armour}, we leverage polynomial zonotopes to compute an overapproximation of the robot's forward occupancy using a set-based formulation of the forward kinematics algorithm.
% Unlike these previous methods, the $\sfo$ is composed of entirely of spheres, which allows efficient distance computatations.

% Next, we discuss how to overapproximates the position of the robot's joints across the family of trajectories using the Spherical Joint Occupancy ($\sjo$).

% Implementing a real-time optimization algorithm to solve this problem is challenging for several reasons.
% First, the constraints associated with obstacle avoidance are non-convex. 
% Second, the constraints must be satisfied for all time $t$ in an uncountable set $T$.
% To address these challenges, a recent paper proposed to represent the trajectory and the forward occupancy of the robot using a polynomial zonotope representation \cite{michaux2023armour}. 
% We summarize these results below. 

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ OLD PZ TRAJ STUFF
% Recall that $\pz{T_i}$ and $\pz{K_j}$ have indeterminates $\tvari$ and $\kjvar$, respectively.

% Because the desired trajectories only depend on $t$ and $k$, the polynomial zonotopes $\pzqji$ and $\pzqdji$  depend only on the indeterminates $\tvari$ and $\kvar$.

% By plugging in a given $k$ for $\kvar$ via the $\setop{slice}$ operation, we obtain a polynomial zonotope where $\tvari$ is the only remaining indeterminate. 

% Because we perform this particular slicing operation repeatedly throughout this document, if we are given a polynomial zonotope, $\pzqdesji$, we use the shorthand $\pzqjki = \setop{slice}(\pzqji, \kvar, k)$.
% The parameterized position and velocity trajectories defined in Def. \ref{defn:traj_param} are functions of both time $t$ and the trajectory parameter $k$.

% Using the time partition $\pz{T_i}$ and trajectory parameter polynomial zonotopes described above, we create polynomial zonotopes $\pzqji$ that overapproximate $\qkj$ for all $t$ in the $i$\ts{th} time subinterval and $k \in K$ by plugging the polynomial zonotopes $\pz{T_i}$ and $\pz{K}$ into the formula for $\qkj$.


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ OLD PZFK STUFF
% The rotation matrix $R\jssmu(q_j(t;k))$ depends on $\cos{(q_j(t;k))}$ and $\sin{(q_j(t;k))}$.
% As a result, we must compute $\cos(\pzqji)$ and $\sin(\pzqji)$ to compute $\pz{R\jssmu}(\pzqji)$.
% Cosine and sine are analytic functions, so we compute  $\cos{(\pzqji)}$ and  $\sin{(\pzqji)}$ using Taylor expansions as in  Sec. \ref{subsec:polyzono}.
% \noindent The Polynomial Zonotope Forward Kinematics Algorithm (PZFK), detailed in Alg. \ref{alg:compose_fk}, is used to compute the objects in Lem. \ref{lem:PZFK} from the set of possible configurations $\pzqi$.


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ OLD SJO STUFF
% \adam{Is it possible this will be confused with the overapproximated joint position trajectories? The terminology in the ARMOUR paper makes it a bit confusing here.
% Or do we want to call it something like spherical joint position occupancy if we include the second part? the first part is really just kinematics, but selecting the position term.}


%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ OLD SLO STUFF
% To describe the links of an arm robot, we utilize tapered capsules described by the convex hull of the two topologically adjacent spheres from the Spherical Joint Occupancy.
% % Thus, the links of the arm robot are described as a collection of joint pairs.
% To ensure a tight overapproximation, these tapered capsules are computed after the center polynomial zonotope is sliced.
% \jon{The \SLO depends on a trajectory parameter $k \in K$.}
% we overappromixate these tapered capsules with overlapping spheres, which we call the spherical forward occupancy
% % This occurs during optimization, where our trajectory parameter $k$ is optimized for and used to slice each joint center polynomial zonotope in $\sfo$.

% % For fast distance querying and computation, we overappromixate these tapered capsules with overlapping spheres, which we call the spherical forward occupancy.
% The spherical forward occupancy is composed of the combination of the spherical joint occupancy and the spherical link occupancy which we will show how to construct.

% we assume that the centers of these sphere are spaced equally apart
% Secondly, to ensure that these spheres fully overapproximate the remaining link volume, we initially construct them such that any two spheres intersect at the surface of the tapered capsule.
% % To simplify the construction of the spherical link occupancy, we assume that we are provided the number of spheres per link, and we assume that the centers of these sphere are spaced equally apart.
% % We do not consider the spherical caps at the ends of the tapered capsule as part of the spherical link occupancy as those are already provided by the spherical joint occupancy.
% Secondly, to ensure that these spheres fully overapproximate the remaining link volume, we initially construct them such that any two spheres intersect at the surface of the tapered capsule.
% We consider a 2D slice of the tapered capsule containing the center line between the defining spheres.
% In this 2D slice, we observe that we can create $n$ isosceles triangles with equivalent base lengths and legs intersecting on the tangent line segment connecting the two circular segments.
% The apex of each isosceles triangle corresponds to each center, and the leg lengths correspond to each respective sphere along the link volume.

% To construct $n$ spheres per link, we want to find the points corresponding to the centers or apex of each triangle, and the radii, or leg lengths of each triangle.
% Since the centers are spaced equally, we can define their distance as odd multiples of $s$.

% \jon{
% \begin{equation}
%     S_{t,j,m} = \text{slice}\left(\mathbf{S}_{t,j,m}\right) = \left(\text{slice}\left((\mathbf{C}_{t,j,m}\right), r_{t,j,m}\right)
% \end{equation}
% \begin{equation}
%     S_{t,j,m} = \text{slice}\left(\mathbf{S}_{t,j,m}\right)
% \end{equation}
% \begin{equation}
%     S_{t,j,m} = \left(c_{t,j,m}, r_{t,j,m}\right)
% \end{equation}
% }


% \jon{\begin{equation}
%     \Delta_{r_{t,j,i}}(k) = \frac{\left(r_{t,j,2} - r_{t,j,1}\right)}{2n}
% \end{equation}
% \begin{equation}
%     \ell_{t,j,i}(k) = r_{t,j,1} + \frac{2i - 1}{2 \ns} \left(r_{t,j,2} - r_{t,j,1}\right)
% \end{equation}}

% \begin{equation}
%     \Delta_{r_{j,i}}(k) = \frac{\left(r_{j+1,i} - r_{j,i}\right)}{2 \ns}
% \end{equation}

% \jon{\begin{equation}
% \theta_{t,j} = \sin^{-1}\left(\frac{r_{t,j,2}-r_{t,j,1}}{\|c_{t,j,2}(k) - c_{t,j,1}(k)\|}\right)
% \end{equation}
% \begin{equation}
% \sprimek = \sk \cdot \cos(\theta_j)
% \end{equation}
% \begin{align*}
% \sprimek^2 &= \sk^2 \cdot \cos^2(\theta_j) \\
%     &= \sk^2 \cdot (1 - \sin^2(\theta_j)) \\
%     &= \sk^2 \cdot \left(1 - \left(\frac{r_{t,j,2}-r_{t,j,1}}{\|c_{t,j,2}(k) - c_{t,j,1}(k)\|}\right)^2\right) \\
%     &= \sk^2 - \left(\frac{r_{t,j,2}-r_{t,j,1}}{2n}\right)^2 \\
%     &= \sk^2 - \Delta_{r_{t,j,i}}(k)^2
% \end{align*}}

% \jon{\begin{equation}
%     \bar{r}_{j,i,m} = \left(\ljmk^2 + \sprimek^2\right)^{\frac{1}{2}}
% \end{equation}
% \begin{equation}
%     \bar{r}_{j,i,m} = \left(\ljmk^2 + \sk^2 - \Delta_{r_{t,j,i}}(k)^2\right)^{\frac{1}{2}}
% \end{equation}}

% \jon{\begin{equation}
%     \cos^2(\alpha) \in [0, 1] \forall \alpha
% \end{equation}
% \begin{equation}
%     \sprimek^2 = \sk^2 \cos^2(\theta_j) \leq \sk^2
% \end{equation}}

% \jon{\begin{align}
%     \bar{c}_{t,j,i} &= c_{t,j,1} + \frac{2i - 1}{2n} \left(c_{t,j,2} - c_{t,j,1}\right) \\
%     \bar{r}_{t,j,i} &= (\ljmk^2 + \sk^2)^{\frac{1}{2}} \\
%     \bar{S}_{t,j,i} &= \left(\bar{c}_{t,j,i}, \bar{r}_{t,j,i}\right)
% \end{align}
% \begin{equation}
%     \slo = \left\{S_{t,j,m}\, : \, \forall t\in T, j\in J, i\in I\right\}
% \end{equation}}
% \begin{equation}
%     \bar{c}_{j,i,m}(k) &= \pzCjik + \frac{2m - 1}{2 \ns} \left(\pz{C_{j+1}}(\pz{T_i}; k) - \pzCjik\right)
% \end{equation}
% \begin{equation}
%     \bar{r}_{j,i,m}(k) &= (\ell_{j,i,m}(k)^2 + s_{j,i}(k)^2)^{\frac{1}{2}} \\
% \end{equation}

% \begin{equation}
%     \Sjik = B(\pzCjik, r_{j,i})
% \end{equation}

% Or for sphere $i$ on link $j$

% \jon{\begin{align}
% \bar{c}_{t,j,i} &= c_{t,j,1} + \frac{2i - 1}{2n} \left(c_{t,j,2} - c_{t,j,1}\right)
% \end{align}}

% With these analytic forms, we are also able to compute jacobians for both the center and radii, which are used during online optimization.

% \begin{equation}
% \theta_j = \sin^{-1}\left(\frac{r_{j,1}-r_{j,2}}{\|p_{j,2}(k) - p_{j,1}(k)\|}\right)
% \end{equation}
% \adam{I'll need to actually verify consistency here because we may have flipped the order of r1 and r2 when doing the on board verification - this is from my own notes}

% \jon{I think the $j$ on the RHS is not the same $j$}
% \begin{align}
% \cjmk &= \pjonek + \frac{2j - 1}{n} (\pjtwok - \pjonek) \\
% \cjmk &= p_j(k) + \frac{2j - 1}{n} (p_{j+1}(k)  - p_j(k) ) 
% \end{align}

% \begin{equation}
%     \rjmk = (\ljmk^2 + \sprimek^2 \cos^2(\theta))^{\frac{1}{2}}
% \end{equation}

% \begin{equation}
%     \sk = \sprimek \cdot \cos(\theta)
% \end{equation}

% \begin{equation}
%     \sprimek = \frac{\|p_{j+1}(k) - p_j(k)\|}{2n}
% \end{equation}
% \jon{feels like we should switch the definition of $\sk$ and $\sprimek$}
% \adam{i agree. when i derived it initially, it was effectively flipped, we just followed this when verifying it on the board.}


% \jon{
% \begin{enumerate}
%     \item This should discuss that each link forward occupancy is a tapered capsule/pill
%     \item We use a finite number of spheres to overapproximate the tapered capsule
%     \item this section discusses how we compute the center and radius of each sphere as a function of our trajectory parameter $k$
%     \item need to define $\theta$
% \end{enumerate}
% }
% To describe the links of an arm robot, we utilize tapered capsules described by the convex hull of the two spheres given by a given link's joint and each of the immediately following joints.
% A given link is thus described as a collection of joint pairs, each of which describe some tapered capsule.
% \adam{This is the more general form, though it seems like we might be making the assumption that we don't have branches? If so, do we want to Keep It Simple?}
% Keep it simple!

% We can over-approximate a given tapered capsule with a fixed number of spheres by choosing sphere centers and radii 



% \begin{equation}
%     % \bar{r}_{j,i,m}(k)  = \left(\ell_{j,i,m}^2 + s_{j,i}(k)^2 - \Delta_{r_{j,i,m}}(k)^2\right)^{\frac{1}{2}}
%      \bar{r}_{j,i,m}(k)  = \left(\ell_{j,i,m}^2 + s_{j,i}(k)^2 - \bigl( \frac{r_{j+1,i} - r_{j,i}}{2 \ns} \bigr)^2 \right)^{\frac{1}{2}}
% \end{equation}

% To find each leg length, we can utilize the Pythagorean theorem on half of the base length and the altitude $l$ of each triangle.
% As the altitude is square to the tangent line, each altitude length corresponds to the interpolated radius for each respective center.


% $s$ also corresponds to the length along the center line which captures half of each isosceles triangle.
% Thus to get half of the base length, we can take the project of this center line to the tangent line.
% We can find this using the following trigonometric relationships.

% Finally, to obtain the leg length:
% However, since theta is small in practice, for online operation we drop this term.
% \begin{equation}
%     \bar{r}_{j,i,m}(k) = (\ell_{j,i,m}^2 + s_{j,i}(k)^2)^{\frac{1}{2}}
% \end{equation}







% %~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ SPHERICAL LINK OCCUPANCY
% \subsubsection{\SLO}\label{subsubsec:slo}
% % \jon{The core of our idea is two parts: 1) we assume that each link is contained in the convex hull of its joint volume overapproximations 2) we only overapproximate the position of the joint frames. }
% Recall from Assum. \ref{assum:joint_link_occupancy} that link $j$ can be outer-approximated by the tapered capsule formed by the two spheres encompassing the closest joints.
% In Sec. \ref{subsubsec:sjo}, we described how to overapproximate each joint volume over a continuous time interval $\pz{T_i}$.
% Therefore, by Assum. \ref{assum:joint_link_occupancy}, the volume occupied by link $j$ over $\pz{T_i}$ is overapproximated by the tapered capsule (Fig. \ref{fig:sfo_2D}) formed by $\Sjik$ and $\Sjpik$ for a given trajectory parameter $k \in K$:
% \begin{equation}
%     \TCjik = \conv(\Sjik \cup \Sjpik) \quad \forall t \in \pz{T_i}.
% \end{equation}

% However, tapered capsules are not ideal for performing collision checking with arbitrary, zonotope-based obstacles.
% Instead, we introduce the \SLO ($\slo$) to overapproximate the volume inside $\TCjik$, but outside $\Sjik$ and $\Sjpik$ using $\ns \in \N$ spheres (Fig. \hyperref[fig:sfo_3D]{3, col. 6}):
% \begin{lem}[Spherical Link Occupancy]\label{lem:slo}
% Let $\TCjik$ be the tapered capsule overapproximation of the $j$\ts{th} link volume at the $i$\ts{th} time step.
% Then for $\ns \in N$ spheres, $\TCjik$ without $\Sjik$ and $\Sjpik$ is overapproximated by the \SLO
% % \begin{equation}\label{eq:tapered_capsule_overapprox}
% %  % \slo(k) \cup \Sjik \cup \Sjpik,
% % % \TCjik \backslash \bigl( \Sjik \cup \Sjpik \bigr) \subset \slo(k)
% % \slok
% % \end{equation}
% % where
% \begin{equation}\label{eq:tapered_capsule_overapprox}
%     \slok = \left\{\Sbarjimk \, : \, \forall j\in \Nq, i\in \Nt, m \in \Ns \right\},
% \end{equation}
% where
% \begin{equation}
%     \Sbarjimk = B\left(\bar{c}_{j,i,m}(k), \bar{r}_{j,i,m}(k)\right),
% \end{equation}
% and 
% for each  $j \in \Nq$,  $k \in \pz{K}$, and $t \in \pz{T_i}$.
% %$\Sjqk \in  \Sjik$
% \end{lem}

% Note that the $\slo$ approximation or  improves as the number of spheres increases.




% %~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ SPHERICAL FORWARD OCCUPANCY
% \subsubsection{Spherical Forward Occupancy}\label{subsubsec:sfo}
% Previous work \cite[Lem. 8]{michaux2023armour} used Lem. \ref{lem:PZFK} along with \eqref{eq:link_occupancy} to overapproximate the forward occupancy of the $j$\ts{th} link over the $i$\ts{th} time step using polynomial zonotopes:
% \begin{align}\label{eq:pz_forward_occupancy_j}
%      \pzFOjKi = \pz{p_j}(\pzqi) \oplus \pz{R_j}(\pzqi)\pz{L_j}.
% \end{align}

% Our key insight is  replacing \eqref{eq:link_occupancy} with an alternate link representation based on a tapered capsule overapproximation of the links \eqref{eq:link_capsule_occupancy}.
% Sections \ref{subsubsec:sjo} and \ref{subsubsec:slo} describe how to overapproximate the swept volume of a link with a collection of spheres.
% Compared to previous methods \cite{holmes2020armtd, michaux2023armour}, our key insight was replacing the link forward occupancy \eqref{eq:link_occupancy} with an approximation based on tapered capsules \eqref{eq:forward_capsule_occupancy}.
% This insight yields a tighter reachable set (Fig. \hyperref[fig:sfo_3D]{3}) compared to previous methods (Fig. \hyperref[fig:sfo]{2F}) while remaining overapproximative. Due to polynomial zonotope operations being exact, or overapproximative, the Spherical Forward Occupancy can be proven to be overapproximative:
% \begin{thm}\label{thm:sfo}
%     The $\sfo$ for link $j$ and time step $t_n$ overapproximates the tapered capsule for link $j$ at time step $t_n$. \jon{finish this theorem}
% \end{thm}

% \input{algorithms/sdf_algorithm}

% \begin{equation}
%     \sfo(k) = \sjo(k)  \cup \slo(k) 
% \end{equation}


% \begin{align}
%     \pz{p_j}(\pzqi) \subset \pzCjiK \oplus B(\mathbf{0}, u_{j,i}) ,
% \end{align}
% \begin{align}
%     \SjiK &= \pzCjiK \oplus B(\mathbf{0}, u_{j,i}) \oplus B(\mathbf{0}, r_j) \nonumber \\
%     &=\pzCjiK \oplus B(\mathbf{0}, r_{j,i}),
% \end{align}
% where $r_{j,i} = r_j + u_{j,i}$.
% Then for all $i \in \Nt$ and $j \in \Nq$ we define the \SJO{} ($\sjo$) as the collection of sets $\SjiK$:
% \begin{equation}
%     \sjo = \left\{\SjiK\, : \, \forall i\in \Nt, j\in \Nq \right\}.
% \end{equation}
% \noindent Note that for any $k \in K$ we can slice each element of $\sjo$ to get a sphere centered at $\pzCjik$ with radius $r_{j,i}$ and the \emph{sliced} \SJO:
% \begin{equation}
%     % \Sjik = B(\pzCjik, r_{j,i}).
%     \Sjik = B(\pzCjik, r_{j,i}).
% \end{equation}
% \begin{equation}
%     \sjo(k) = \left\{\Sjik\, : \, \forall i\in \Nt, j\in \Nq \right\}.
% \end{equation}

==> sections/05_demonstrations.tex <==
\section{Demonstrations}\label{sec:demonstrations}
We demonstrate \methodname in simulation using the Kinova Gen3 7 DOF manipulator.
Code, data, and video demonstrations can be found at \url{https://roahmlab.github.io/sparrows/}.

%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ IMPLEMENTATION DETAILS
\subsection{Implementation Details}
Experiments for \methodname, \armtd \cite{holmes2020armtd}, and \mpot \cite{le2023mpot} were conducted on a computer with an Intel Core i7-8700K CPU @ 3.70GHz CPU and two NVIDIA RTX A6000 GPUs. 
Baseline experiments for \chomp \cite{Zucker2013chomp} and \trajopt \cite{Schulman2014trajopt} were conducted on a computer with an Intel Core i9-12900H @ 4.90GHz CPU.
Polynomial zonotopes and their arithmetic are implemented in PyTorch \cite{paszke2017automatic} based on the CORA toolbox \cite{cora2018}.

\subsubsection{Simulation and Simulation Environments}
% We use the Kinova Gen3 7-DOF serial manipulator \cite{kinova-user-guide} and place its base at the origin of each simulation environment.
We use a URDF of the Kinova Gen3 7-DOF serial manipulator \cite{kinova-user-guide} from \cite{kinovakortex} and place its base at the origin of each simulation environment.
Collision geometry for the robot is provided as a mesh, which we utilize with the trimesh library \cite{trimesh} to check for collisions with obstacles. 
Note that we do not check self-collisions of the robot.
% The collision geometry of each of Kinova's link is represented as the smallest bounding box enclosing the native link geometry.
% \adam{The collision geometry for each Kinova link is represented as teh smallest bounding box enclosing the native link geometry.(?) Also, we do mesh-based collision after this, so collision checks aren't purely based on bounding-box (unless qingyi did set it to use bounding boxes).}\qc{collision are checked by mesh indeed}
For simplicity, all obstacles are static, axis-aligned cubes parameterized by their centers and edge lengths. 
We assume that the start and goal configurations of the robot are collision-free. Although we do not assume that a feasible path exists in each environment, most scenes were determined to be feasible by running an RRT \cite{LaValle1998rrt} for several minutes.
%\jon{@adam @qc can you clean this bit of the paper up?}
\subsubsection{Signed Distance Computation}
Recall from Assum. \ref{assum:env} that each obstacle is represented by a zonotope $Z$.
The edges $E$ and polytope representation $(A,b)$ of $Z$ are computed offline before planning begins.
PyTorch is used to build the computation graph for calculating the signed distances in Alg. \ref{alg:sdf}.
The analytical gradients of the output of Alg. \ref{alg:sdf} are derived and implemented to speed up the optimization problem \optref.

\subsubsection{Desired Trajectory}
We parameterize the trajectories with a piece-wise linear velocity such that the
 \defemph{trajectory parameter} $k=(k_1,\cdots,k_{\nq})\in\R^{\nq}$ is a constant acceleration over the planning horizon $[0, \tplan)$.
The trajectories are also designed to contain a constant braking acceleration applied over $[\tplan, \tfin]$ that brings the robot safely to a stop.
Thus, given an initial position $q_{0}$ and velocity $\dot{q}_{0}$, the parameterized trajectory is given by:
\begin{align}\label{eq:actual_trajectory}
    q(t;k) = \begin{cases}
        q_0 + \dot{q}_0t + \frac{1}{2}k\,t^2, &t \in [0,\tplan) \\
        q_0 + \dot{q}_0\tplan + \frac{1}{2}k\,\tplan^2 + \\ (\dot{q}_0\tplan + k\tplan)\frac{(2\tfin-\tplan-t)(t-\tplan)}{2(\tfin - \tplan)}, &t \in [\tplan,\tfin].
    \end{cases}
\end{align}


\subsubsection{Optimization Problem Implementation}
\methodname{} and \armtd{} utilize IPOPT \cite{ipopt-cite} for online planning by solving \optref.
The constraints for \optref, which are constructed from the \SJO (Lem. \ref{lem:sjo}) and \SFO (Thm. \ref{thm:sfo}), are implemented in PyTorch using polynomial zonotope arithmetic based on the CORA toolbox \cite{cora2018}.
All of the constraint gradients of \optref{} were computed analytically to improve computation speed.
Because polynomial zonotopes can be viewed as polynomials, all of the constraint gradients can be readily computed using the standard rules of differential calculus.

\subsubsection{Comparisons}
We compare \methodname to \armtd \cite{holmes2020armtd} where the reachable sets are computed with polynomial zonotopes similar to \cite{michaux2023armour}.
We also compare to \chomp \cite{Zucker2013chomp}, \trajopt \cite{Schulman2014trajopt}, \curobo \cite{sundaralingam2023curobo}, and \mpot \cite{le2023mpot}.
We used the ROS MoveIt \cite{moveit2014} implementation for \chomp, Tesseract Robotics's ROS package \cite{tesseracttrajopt} for \trajopt, and the original implementation for \mpot \cite{le2023mpot}.
%\adam{cite this: https://github.com/tesseract-robotics/trajopt}
Note that \mpot's signed distance function was modified to account for the obstacles in the planning tasks we present here.
Although \chomp, \trajopt, \curobo, and \mpot are not receding-horizon planners, each method provides a useful baseline for measuring the difficulty of the scenarios encountered by \methodname.
Note that for simplicity, we do not consider self-intersection constraints for \methodname or any of the baseline methods.
We also include a detailed discussion in App. \ref{app:ablation} on how the parameters in each of the baseline methods were tuned.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/hard_scenarios.pdf}
    \caption{Subset of \textbf{Realistic Scenarios} where \methodname succeeds.
    The start, goal, and intermediate poses are shown in blue, green, and grey (transparent), respectively. 
    Obstacles are shown in red (transparent).
    The tasks include reaching from one side of a wall to another, between two small bins, from below to above a shelf, around one vertical post, and between two horizontal posts. 
    Video demonstrations can be found at \url{https://roahmlab.github.io/sparrows/}.
    }
    \label{fig:hard_scenarios}
\end{figure*}
%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ RESULTS
\subsection{Runtime Comparison with \armtd}
\input{tables/mean_runtime}
\input{tables/avg_planning_time}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.93\columnwidth]{figures/acceleration_comparison_q.pdf}
    \caption{A comparison of \methodname' and \armtd's reachable sets. 
    (Top row) Both \methodname and \armtd can generate trajectories that allow the arm to fit through a narrow passage when the maximum acceleration is limited to $\frac{\pi}{24}$ rad/s$^2$. 
    (Bottom row) However, when the maximum acceleration is $\frac{\pi}{6}$ rad/s$^2$ \armtd's reachable set collides with the obstacles while \methodname' remains collision-free.}
    \label{fig:reachset_comparison}
    \vspace*{-0.3cm}
\end{figure}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth/3]{figures/baselines10.png}%
    \includegraphics[width=\textwidth/3]{figures/baselines20.png}%
    \includegraphics[width=\textwidth/3]{figures/baselines40.png}    
    \caption{\textbf{Grid of Baseline Comparison Timelapses.} A subset of \textbf{Random Obstacle Scenarios} where \methodname succeeds and all other methods fail. 
    The start, goal, and intermediate poses are shown in blue, green, and grey (transparent), respectively. 
    Obstacles are shown in red (transparent).
    The columns, ordered from left to right, correspond to scenes with 10, 20, and 40 obstacles. 
    (Row 1) \methodname. (Row 2) \armtd. (Row 3) \trajopt. (Row 4) \mpot. (Row 5) \curobo.
    Video demonstrations for each of these runs can be found in the accompanying supplementary material.
    }
    \label{fig:baseline_grid}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/14dof_timelapse.png}
    \caption{A 14 DOF demonstration from the \textbf{Random Obstacle Scenarios} where \methodname succeeds.
    The start, goal, and intermediate poses are shown in blue, green, and grey (transparent), respectively. 
    Obstacles are shown in red (transparent).
    A video demonstration can be found in the accompanying supplementary material.
    }
    \label{fig:timelapse14dof}
    \vspace*{-0.5cm}
\end{figure*}
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\textwidth]{figures/21dof_timelapse.png}
    \caption{A 21 DOF demonstration from the \textbf{Random Obstacle Scenarios} where \methodname succeeds.
    The start, goal, and intermediate poses are shown in blue, green, and grey (transparent), respectively. 
    Obstacles are shown in red (transparent).
    A video demonstration can be found in the accompanying supplementary material.
    }
    \label{fig:timelapse21dof}
    \vspace*{-0.5cm}
\end{figure*}
% We compare the runtime performance of \methodname{} to \armtd{} while varying the number of obstacles, maximum acceleration, planning time limit, and the degrees of freedom of the robot.
We compare the runtime performance of \methodname{} to \armtd{} while varying the number of obstacles, maximum acceleration, and planning time limit.
We measure the mean constraint evaluation time and the mean planning time.
Constraint evaluation includes the time to compute the constraints and the constraint gradients.
Planning time includes the time required to construct the reachable sets and the total time required to solve \optref{} including constraint gradients evaluations.
We consider planning scenarios with $n=10$, $20$, and $40$ obstacles each placed randomly such that each obstacle is reachable by the end effector of the robot.
% We consider planning scenarios with $n=5$, $10$, $20$, and $40$ obstacles each placed randomly such that each obstacle is reachable by the end effector of the robot.
We also consider two families of parameterized trajectories \eqref{eq:actual_trajectory} such that the maximum acceleration is $\pi/24$ rad/s$^2$ or $\pi/6$ rad/s$^2$, respectively.
The robot is allowed to have $7$, $14$, or $21$ degrees of freedom by having 1, 2, or 3 Kinova arms in the environment.
The maximum planning time is limited to $0.15$s, $0.25$s, or $0.5$s for the $7$ DOF arm and $0.5$s and $1.0$s for the $14$ and $21$ DOF arms.
For each case, the results are averaged over 100 trials.


Tables \ref{tab:consevalruntime3d7link0.5s} and \ref{tab:planningtime3d7link0.5s} summarize the results for a $7$ DOF robot with a $0.5$s planning time limit.
\methodname$(\pi/24)$ has the lowest mean constraint evaluation time and per-step planning time followed by \methodname$(\pi/6)$. 
For each maximum acceleration condition, \methodname' average planning time is almost twice as fast as \armtd when there are 20 or more obstacles.
Note that we see a similar trend when the planning time is limited to $0.25s$ and $0.15s$.
Further note that under planning time limits of $0.25$s (Table \ref{tab:consevalruntime3d7link0.25s}) and $0.15$s (Table \ref{tab:consevalruntime3d7link0.15s}), \armtd is unable to evaluate the constraints quickly enough to solve the optimization problem within the allotted time as the number of obstacles increases (Table \ref{tab:consevalruntime3d7link0.25s}). 
This is consistent with the cases when \armtd's mean planning time limit exceeds the maximum allowable planning time limits in Tables \ref{tab:planningtime3d7link0.5s}, \ref{tab:planningtime3d7link0.25s}, and \ref{tab:planningtime3d7link0.15s}.

\input{tables/spharmour_vs_armtd_multiarm}
Tables \ref{tab:multiarm_planningtime_1.0s} and \ref{tab:multiarm_consevaltime_1.0s} present similar results for robots with $14$ and $21$ degrees of freedom.
Similar to the previous results, \methodname computes the constraints and constraint gradients almost twice as fast as \armtd.
Furthermore, compared to \methodname, \armtd struggles to generate motion plans in the allotted time.


% \begin{figure*}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{figures/hard_scenarios.pdf}
%     \caption{Subset of Hard Scenarios where \methodname succeeds.
%     The start, goal, and intermediate poses are shown in blue, green, and grey (transparent), respectively. 
%     Obstacles are shown in red (transparent).
%     The tasks include reaching from one side of a wall to another, between two small bins, from below to above a shelf, around one vertical post, and between two horizontal posts. }
%     \label{fig:hard_scenarios}
% \end{figure*}




\subsection{Motion Planning Experiments}\label{subsec:baselines}
% We compare the performance of \methodname to \armtd, \chomp, \trajopt, and \mpot on two sets of scenarios.
We evaluate the performance of \methodname{} on two sets of task scenes.
The first set of scenes, \textbf{Random Obstacle Scenarios}, shows that \methodname can generate safe trajectories for arbitrary tasks and DOFs.
For the $7$ DOF tasks, the scene contains a single Kinova arm with arm, the scene contains $n_{\mathcal{O}}=10$, $20$, or $40$ axis-aligned boxes that are $20$cm on each side.
For the $14$ and $21$ DOF tasks, the scene contains 2 or 3 Kinova arms treated as a single robot with arms, the scene contains $n_{\mathcal{O}}=5$, $10$, or $15$ obstacles of the same size.
% \adam{We refer to this subset for the $14$ and $21$ DOF arms as \textbf{Multi-arm Random Obstacle Scenarios}}
For each number of obstacles, we generate 100 task scenes with obstacles placed randomly such that the start and goal configurations are collision-free.
Note that a solution to the goal may not be guaranteed to exist.
The second set of tasks, \textbf{Realistic Scenarios}, contains 14 tasks with a Kinova arm and the number of obstacles varying from $5$ to $20$.
The \textbf{Realistic Scenarios} show that \methodname can generate safe trajectories in scenes containing geometric features similar to those found in a household setting. 
We compare the performance of \methodname to \armtd, \chomp, \trajopt, and \mpot on both sets of scenarios for the $7$ DOF arm.
We further compare the performance of \methodname to \armtd on Random Obstacle Scenarios for the $14$ and $21$ DOF robots.

% In all tests, \methodname and \armtd are given planning time limits of $t_p=0.15$s, $0.25$s, and $0.5$s a maximum of 150 planning iterations to reach the goal 
In the tests with a $7$ DOF arm, \methodname and \armtd are given a planning time limit of $0.5$s and a maximum of 150 planning iterations to reach the goal. For the tests with $14$ and $21$ DOF robots, \methodname and \armtd are given a planning time limit of $1.0$s and a maximum of 150 planning iterations. 
We imposed a planning time limit of 100s, 30s, and 2s on \chomp{}, \trajopt{}, and \curobo{}, respectively.
These planning time limits were chosen such that the max planning time limit was greater than 5x the average planning time to solve the sample set of random problems that were drawn from our experimental setup.
We include additional results for the average planning times for the baseline methods in Table \ref{tab:planning_time_stats_baseline}.

A failure occurs if \methodname or \armtd fails to find a plan for two consecutive planning iterations or if a collision occurs.
Note that meshes for the robot and obstacles are used to perform ground truth collision checking within the simulator.
% Finally, \methodname and \armtd are given a straight-line high-level planner for the Random Obstacles scenarios and the Hard Scenarios are given waypoints generated by RRT$^*$ \cite{karaman2011rrtstar}.
% \jon{Remove the RRT experiments.} \qc{Finally, \methodname and \armtd are given a straight-line high-level planner for both the Random Obstacles scenarios and the Hard Scenarios.}
Finally, \methodname and \armtd are given a straight-line high-level planner for the \textbf{Random Obstacle Scenarios} and \textbf{Realistic Scenarios}.

Table \ref{tab:random_obstacles_0.5s} presents the results for the $7$ DOF \textbf{Random Obstacle Scenarios} where \methodname and \armtd are given a maximum planning time limit $0.5$s.
\methodname ($\pi/6$) achieves the highest success rate across all obstacles followed by \methodname $(\pi/24)$. 
A representative example is shown in Fig. \ref{fig:baseline_grid}.
Notably, the performance of \armtd degrades drastically as the number of obstacles is increased.
This is consistent with \armtd's slower constraint evaluation presented in Table \ref{tab:consevalruntime3d7link0.5s}, \armtd's mean planning time exceeding the limit, and \armtd's overly conservative reachable sets shown in Fig \ref{fig:reachset_comparison}.
Although \armtd remains collision-free, these results suggest that the optimization problem is more challenging for \armtd to solve.
In contrast \chomp, \trajopt, and \mpot exhibit much lower success rates.
Note that \trajopt and \mpot frequently crash whereas \chomp does not return feasible trajectories.
% Note that we observe a similar trend when the planning time is limited to $0.25$s or $0.15$s

Table \ref{tab:multiarm_success1.0} compares the success rate of \methodname to \armtd on \textbf{Random Obstacle Scenarios} for higher degrees of freedom.
Representative planning scenarios are shown in Fig. \ref{fig:timelapse14dof} and Fig. \ref{fig:timelapse21dof}.
For $14$ degrees of freedom and $n_{\mathcal{O}} = 5$ obstacles, \armtd$(\pi/24)$ has more successes, though \mbox{\methodname$(\pi/24)$} and \methodname$(\pi/6)$ remain competitive.
Note, in particular, that \methodname $(\pi/6)$'s success rate is more than double that of \armtd $(\pi/6)$ for $10$ and $15$ obstacles.
For $21$ degrees of freedom, the performance gap between \methodname and \armtd is much larger as \armtd fails to solve any task in the presence of $10$ and $15$ obstacles.

Table \ref{tab:hard_scenarios_0.5s} presents results for the \textbf{Realistic Scenarios} (Fig. \ref{fig:hard_scenarios}). 
\chomp outperforms all baseline methods with 10 successes, followed by \mpot which obtains 6 successes and 5 collisions.
\chomp's success rate of $71\%$ on the \textbf{Realistic Scenarios} is similar to its success rate on the \textbf{Random Obstacles Scenarios} for $n=10$ obstacles.
This is likely due to \chomp's ability to generate motion plans when the obstacle density is low.
Notably, \chomp also outperforms \methodname$(\pi/6)$ which is the best-performing method on the \textbf{Random Obstacles Scenarios}.
By design, \methodname and \armtd are both receding-horizon trajectory planners that may behave myopically when optimizing for a single path to reach the next waypoint.
Thus, both methods can get stuck in local minima without a good high-level planner.
This is in contrast to the baseline methods which all optimize for the entire plan.
To test this, we evaluated the performance of \methodname$(\pi/6)$ and \armtd$(\pi/6)$ on the \textbf{Realistic Scenarios} when given access to a high-level planner.
Table \ref{tab:hard_scenarios_0.5s} shows that \methodname$(\pi/6) + \text{HLP}$ can successfully solve all of the tasks when using a high-level planner, whereas \armtd$(\pi/6) +\text{HLP}$ is only able to solve 8 of the tasks.
Note that no assumptions were made on the safety of waypoints given by the high-level plan.

\input{tables/baseline_comparisons}




% \subsubsection{Single Arm Planning}
% \label{subsec: simulation}

% \begin{itemize}
%     \item \jon{For our random scenes, our obstacles were chosen to have a side-length of 20cm with minimum distance of 1cm from the start or end configuration when generated.}
%     % \item we run each method on 100 trials of same scenarios. Note that \methodname{} and \armtd{} are using pi/24 as the k-range.
%     % \item we report their \# success (and \# collision) under various \# obs and time limits in table \ref{tab:success3d7link24pi}
%     \item we report their mean planning time under 0.5s time limit in table \ref{tab:time3d7link24pi}
%     \item we run \methodname{} and \armtd on 100 trials of same scenarios. 
%     Note that we are using pi/6 as the k-range this time. This allows the robot to have larger acceleration/deceleration but also leads to larger reachset.
%     \item we report their \# success (no collision occurred) under various \# obs and time limits in table \ref{tab:success3d7link6pi}
%     \item we report their mean planning time under 0.5s time limit in table \ref{tab:time3d7link6pi}
%     \item At the start of every planning trial, we randomize collision-free start and end configurations for the arm.
%     % \item Obstacle positions are sampled such that each obstacle is within reach of the arm.
%     \item We also repeat these experiments using various time limits to test their 
% \end{itemize}
% \begin{itemize}
%     \item \jon{where to discuss how we choose a size for the joint spheres of the nominal joint spheres?}
%     \item \jon{where to discuss how we chose the number of spheres?}
% \end{itemize}

%  \subsubsection{Multi-Arm Planning}
% \begin{itemize}
%     \item we run \methodname{} and \armtd{} with 2 and 3 kinova arms. This leads the DOF of the system to be 14 and 21, respectively. We use pi/6 as the k-range. 
%     \item we report their \# success (no collision occurred) under various \# obs and time limits in table \ref{tab:success3d14link6pi}
%     \item we report their mean planning time under 0.5s time limit in table \ref{}
% \end{itemize}

%\input{tables/spharmour_vs_armtd_multiarm}
% Note that the larger acceleration allows the robot to have larger acceleration/deceleration but also leads to larger reachset.
%\input{tables/multiarm}

% \begin{itemize}
%     \item \jon{Is it worth discussing the multi-arm experiments if we didn't do the same amount of analysis?}
% \end{itemize}

==> sections/approach.tex <==
\section{Reachability-based Signed Distance Function}\label{sec:approach}

\subsection{Signed Distance Between Zonotopes}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/buffer_obstacle.pdf}
    \caption{Illustration of signed distance for convex polytopes. In particular, this works well with zonotopes.\jon{Add labels. Highlight pos/neg distance better.}} 
    \label{fig:zono_sdf}
    \vspace*{-0.2cm}
\end{figure}
In this section we describe how to compute signed distance between two zonotopes, how to represent this function exactly using a ReLU neural network, and how we leverage this novel representation for representing obstacle-avoidance constraints for safe motion planning.

\begin{defn}\label{defn:zono_pentration_depth}
    The \defemph{penetration depth} of $Z_1$ and $Z_2$ in $\R^{\nd}$ is denoted $\pi(Z_1, Z_2)$ and is defined by 
    \begin{equation}
        \pdf(Z_1, Z_2) = \min \{\|t\| :\ \text{int}(Z_1 + t \cap Z_2) = \emptyset, \quad t \in \R^{\nd}\}.
    \end{equation}
\end{defn}


\begin{lem}\label{lem:zono_sdf}
Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes such that $Z_1 \cap Z_2 \neq \emptyset$. 
Then the signed distance between $Z_1$ and $Z_2$ is given by
\begin{equation}
    \sdf(Z_1, Z_2)  = 
        \begin{cases}
          \dist(c_1; Z_{2,buf})  & \text{if } c_1 \not \in Z_{2,buf} \\
          -\pdf(c_1, Z_{2,\text{buf}}) & \text{if } c_1 \in Z_{2,buf}
        \end{cases} .
\end{equation}
\end{lem}
\begin{proof} See \cite{michaux2023rdf}.
\end{proof}

Maybe say something about how this can be solved using a convex optimization program.
But here, we instead compute the distances exactly.


\begin{lem} \label{lem:hyperplane_distance}
We can compute the distance  
\end{lem}
\begin{proof} Let 
\begin{equation}
    h_i(t) = v_1 + s (v_2 - v_1) 
\end{equation}
for $s \in [0,1]$.

The distance between a point and the line segment is
\begin{equation}
    \phi_i(s) = \|h_i(s) - p\|^2
\end{equation}

\begin{equation}
    \hat{s}_i = \frac{(p - v_1)^T(v_2 - v_1)}{(v_2 - v_1)^T (v_2 - v_1)}
\end{equation}

\begin{equation}
    s^{\ast}_i = \min (\max (\hat{s}_i, 0), 1)
\end{equation}
\end{proof}

\begin{thm} \label{thm:exact_sdf}
The distance between two zonotopes can be computed
\end{thm}
\begin{proof}
\end{proof}
Note that we provide a visual illustration of this theorem in Fig. \ref{fig:zono_sdf}.
We use this to build the neural network in the next section
\subsection{Neural Network Architecture}

\begin{thm}
\label{thm:network_bound}
\end{thm}
\begin{proof}
\end{proof}


% Before proving the required result, we prove several intermediate results. 
% \subsection{Signed Distance Between Zonotopes}
% \label{subsec:sdf_zono}

% Here we derive the signed distance between two zonotopes.
% To proceed we first require a condition for determining if two zonotopes are in collision:
% \begin{lem}\label{lem:zono_intersection}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes. Then $Z_1 \cap Z_2 \neq \emptyset$ if and only if $c_1 \in Z_{2,\text{buf}} = (c_2, G_1 \cup G_2)$.
% \end{lem}
% \begin{proof}
% Suppose the intersection of $Z_1$ and $Z_2$ is non-empty. This is equivalent to the existence of $z_1 \in Z_1$ and $z_2 \in Z_2$ such that $z_1 = z_2$. Furthermore, by definition of a zonotope (Defn. \ref{defn:zonotope}), this is equivalent to the existence of coefficients $\beta_1$ and $\beta_2$ such that $z_1 = c_1 + G_1 \beta_1$, $z_2 = c_2 + G_2 \beta_2$, and
% \begin{align}
%     &c_1 + G_1 \beta_1 = c_2 + G_2 \beta_2 \\
%     \iff& c_1 = c_2 + G_2 \beta_2 - G_1 \beta_1 \\
%     \iff& c_1 \in (c_1, G_1 \cup G_2) = Z_{2, \text{buf}}.
% \end{align}
% Thus we have shown that $Z_1 \cap Z_2 \neq \emptyset$ if and only if $c_1 \in (c_1, G_1 \cup G_2) = Z_{2, \text{buf}}$.
% \end{proof}

% Lemma \ref{lem:zono_intersection} can then be used to compute the the positive distance between two non-intersecting zonotopes:
% \begin{lem}\label{lem:zono_positive_distance}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be non-intersecting zonotopes.
% \begin{align}
%     \dist(Z_1, Z_2) = \dist(c_1; Z_{2,buf})
% \end{align}
% where $Z_{2,\text{buf}} = (c_2, G_1 \cup G_2)$.
% \end{lem}
% \begin{proof}
% Suppose $Z_1$ and $Z_2$ are non-intersecting zonotopes such that $\dist(Z_1, Z_2) = r$ for some $r \in \mathbb{R}^{+}$. That is, there exists $z_1 \in Z_1$ and $z_2 \in Z_2$ such that 
% \begin{align}
%     r &= \|z_1 - z_2\| \\
%     &= \|c_1 + G_1 \beta_1 - (c_2 + G_2 \beta_2) \| \\
%     &= \| c_1 - (c_2 + G_2 \beta_2 = G_1 \beta_1) \| \\
%     &\geq \dist(c_1, (c_2, G_1 \cup G_2)) \\
%     &= \dist(c_1, Z_{2, \text{buf}}).
% \end{align}
% Now suppose $\dist(c_1, Z_{2, \text{buf}}) = r$. Then there exists coefficients $\beta_1$ and $beta_2$ such that
% \begin{align}
%     r &= \|c_1 - (c_2 + G_1 \beta_1 + G_2 \beta_2) \| \\
%     &= \|c_1 - G_1 \beta_1 - (c_2 + G_2 \beta_2) \| \\
%     &= \|z_1 - z_2\| \\
%     &\geq \dist(Z_1, Z_2).
% \end{align}
% Together, these inequalities prove that $\dist(Z_1, Z_2) = \dist(c_1; Z_{2,buf})$.
% \end{proof}
% Let $\text{int}(S)$ denote the interior of a set.
% Before deriving the negative distance we first define the penetration depth  \cite{cameron1986mtd} of two zonotopes:
% \begin{defn}\label{defn:zono_pentration_depth}
%     The \defemph{penetration depth} of $Z_1$ and $Z_2$ in $\R^{\nd}$ is denoted $\pi(Z_1, Z_2)$ and is defined by 
%     \begin{equation}
%         \pdf(Z_1, Z_2) = \min \{\|t\| :\ \text{int}(Z_1 + t \cap Z_2) = \emptyset, \quad t \in \R^{\nd}\}.
%     \end{equation}
% \end{defn}

% The penetration depth $\pi(Z_1,Z_2)$ can be interpreted as the minimum translation applied to $Z_1$ such that the interior of $Z_1 \cap Z_2$ is empty.
% Following \cite{agarwal2000convex} we can now redefine the penetration distance between $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ in terms of $c_1$ and $Z_{2,\text{buf}}$.
% \begin{lem}\label{lem:zono_negative_distance}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes such that $Z_1 \cap Z_2 \neq \emptyset$.
% Then the penetration depth between $Z_1$ and $Z_2$ is given by
%    \begin{align}
%      \pdf(Z_1, Z_2) = \pi(c_1, Z_{2,\text{buf}}),
% \end{align} 
% \end{lem}
% \begin{proof}
% Suppose $Z_1 \cap Z_2 \neq \emptyset$. 
% Then by Defn. \ref{defn:zono_pentration_depth}, there exists a translation vector $t \in \R^{\nd}$ such that $\text{int}(Z_1 + t \cap Z_2) = \emptyset$. 
% This means that $Z_1$ is translated by $t$ such that only the boundaries of $Z_1 + t$ and $Z_2$ are intersecting. 
% Thus, there exists $z_1 \in \partial Z_1$ and $z_2 \in \partial Z_2$ such that $z_1 + t = z_2$. 
% Furthermore, there exist coefficients $\beta_1$ and $\beta_2$ such that $z_1 = c_1 + G_1 \beta_1$, $z_2 = c_2 + G_2 \beta_2$, and
% \begin{align}
%     & c_1 + G_1 \beta_1 + t = c_2 + G_2 \beta_2 \\
%     \iff& c_1 + t = c_2 + G_2 \beta_2 - G_1 \beta_1 \in \partial Z_{2,\text{buf}}.
% \end{align}
% Since $\pi(c_1, Z_{2,\text{buf}})$ is the minimum distance between $c_1$ and all points in $\partial Z_{2,\text{buf}}$, this means that $\pi(c_1, Z_{2,\text{buf}}) \leq \|t\|$.

% Now suppose $c_1 \in Z_{2, \text{buf}}$.
% Let $t \in \R^{\nd}$ such that $\|t\|$ is the penetration depth of $c_1$ and $Z_{2,\text{buf}}$. 
% Then there exists coefficients $\beta_1$ and $\beta_2$ such that $z_2 = c_2 + G_1 \beta_1 + G_2 \beta_2$ and
% \begin{align}
%     c_1 + t = c_2 + G_1 \beta_1 + G_2 \beta_2 \\
%     c_1 -G_1 \beta_1 + t = c_2 + G_2 \beta_2.
% \end{align}
% This means translating $z_1 = c_1 - G_1 \beta_1 \in \partial Z_1$ by $t$ causes the boundary of $Z_1$ to intersect the boundary of $Z_2$. 
% Therefore $\pi(Z_1, Z_2) \leq \|t\|$.
% Together the above inequalities prove the result.
% \end{proof}

% \begin{thm}\label{thm:zono_sdf}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes such that $Z_1 \cap Z_2 \neq \emptyset$. 
% % Denote $\mathcal{P} = \bigcap_{i}\mathcal{H}_i$ as the half-space representation of the buffered zonotope $Z_{2,buf} = (c_2, G_1 \cup G_2)$.
% Then the signed distance between $Z_1$ and $Z_2$ is given by
% \begin{equation}
%     \sdf(Z_1, Z_2)  = 
%         \begin{cases}
%           \dist(c_1; Z_{2,buf})  & \text{if } c_1 \not \in Z_{2,buf} \\
%           -\pdf(c_1, Z_{2,\text{buf}}) & \text{if } c_1 \in Z_{2,buf}
%         \end{cases} .
% \end{equation}
% \end{thm}
% \begin{proof} The proof follows readily from Lemmas \ref{lem:zono_positive_distance} and \ref{lem:zono_negative_distance}.
% \end{proof}

% Note that we provide a visual illustration of this theorem in Fig. \ref{fig:zono_sdf}.

% \subsection{The Proof}

% We prove the desired result by considering two cases. 
% First assume  $O \cap \FO(q(T;k)) = \emptyset$ for all $t \in T$. 
% Then
% \begin{align}
%     \rdf(O, \FO(q(T;k))) &= \underset{t \in T}{\min}\: \underset{j \in \Nq}{\min}\:  \sdf(O, \FO_j(q(t;k))) \\
%     &\geq \underset{i \in \Nt}{\min}\: \underset{j \in \Nq}{\min}\:  \sdf(O, \pzFOjki) \\
%     % &= \underset{i \in \Nt}{\min}\: \underset{j \in \Nq}{\min}\: \sdf(O, \pzFOjkibuf) \\
%     &= \underset{i \in \Nt}{\min}\: \underset{j \in \Nq}{\min}\: \sdf(\co, \pzFOjkibuf) \\
%     &= \underset{j \in \Nq}{\min}\: \sdf(\co, \bigcup_{i\in\Nt} \pzFOjkibuf) \\
%     &\geq \underset{j \in \Nq}{\min}\: \sdf(\co, \Pj) \\
%     &= \underset{j \in \Nq}{\min}\: \ardf_j(\co, \Pj) \\
%     &= \ardf(\co, \bigcup_{j\in \Nq} \Pj),
% \end{align}
% where the first equality follows from the definition of $\rdf$ in Def. \ref{def:rdf_point}, the second inequality follows from Lemma \ref{lem:pz_FO}, the third equality follows from Lemma \ref{lem:zono_positive_distance}, the fourth inequality by flipping the order of minimization, and the fifth inequality follows from Def. \ref{def:convhull}. 

% Thus $\ardf$ underapproximates the distance between the forward occupancy and the obstacle. 
% If instead $O \cap \FO_j(\q) \neq \emptyset$ for some $t \in T$, replacing $\geq$ with $\leq$ shows that we can overapproximate the penetration distance between an obstacle and the forward occupancy.

% \begin{lem}\label{lem:zono_negative_distance}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes such that $Z_1 \cap Z_2 \neq \emptyset$. Denote $\mathcal{P} = \bigcap_{i}\mathcal{H}_i$ as the half-space representation of the buffered zonotope $Z_{2,buf} = (c_2, G_1 \cup G_2)$. Then the penetration depth of $Z_1$ and $Z_2$ is
%    \begin{align}
%      \pi(Z_1, Z_2) = \underset{i}{\min}\:\dist(c_1, \mathcal{H}_i),
% \end{align} 
% where $\mathcal{P}$ is the polytope representation of $Z_{2,buf} = (c_2, G_1 \cup G_2)$.
% \end{lem}
% \begin{proof}
%     See Appendix.
%     % It is readily apparent that
%     % \begin{align}
%     %     \pi(Z_1, Z_2) = \pi(c_1, Z_{2,buf}).
%     % \end{align}
% \end{proof}


\subsection{Algorithm}
\input{algorithms/redefine_alg}
\begin{itemize}
    \item Will probably want to 
\end{itemize}


==> sections/clean_abstract.tex <==
Safe motion planning algorithms are necessary for deploying autonomous robots in unstructured environments.  Motion plans must be safe to ensure that the robot does not harm humans or damage any nearby objects. Generating these motion plans in real-time is also important to ensure that the robot can adapt to sudden changes in its environment. Many trajectory optimization methods introduce heuristics that balance safety and real-time performance, potentially increasing the risk of the robot colliding with its environment. This paper addresses this challenge by proposing Conformalized Reachable Sets for Obstacle Avoidance With Spheres (CROWS). CROWS is a novel real-time, receding-horizon trajectory planner that generates probablistically-safe motion plans. Offline, CROWS learns a novel neural network-based representation of a sphere-based reachable set that overapproximates the swept volume of the robot's motion. CROWS then uses conformal prediction to compute a confidence bound that provides a probabilistic safety guarantee on the learned reachable set. At runtime, CROWS performs trajectory optimization to select a trajectory that is probabilstically-guaranteed to be collision-free. We demonstrate that CROWS outperforms a variety of state-of-the-art methods in solving challenging motion planning tasks in cluttered environments while remaining collision-free. Code, data, and video demonstrations can be found at \url{https://roahmlab.github.io/crows/}.

==> sections/old/06_network.tex <==
\section{Exact SDF with ReLU Networks}




















%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ OLD STFF


\label{sec:nnsdf}
The Section \ref{sec:sfo} described how to construct the .
Because this representation is composed of spheres, it is straightforward to use with a signed distance function.
This section first describes how to compute the signed distance function exactly between a zonotope and a point in 3D. between two zonotopes, how to represent this function exactly using a ReLU neural network, and how we can replace the obstacle-avoidance constraints in \opt with a novel neural implicit representation that overapproximates the distance between the forward occupancy of the ego vehicle and obstacles in the environment.



\subsection{Exact Signed Distance Between a Point and a Zonotope}
\label{subsec:rdf_derivation}
% We start by stating a result about the signed distance between two zonotopes: \jinsun{Pls use calligraphic font for sets...}
% \jon{Why?}

% \begin{lem}\label{lem:zono_sdf}
% Let $Z = (\cz, \Gz)$ and $O = (\co, \Go)$ be zonotopes and define $\Oz = (\cz, \Gz \cup \Go)$ \jinsun{$\Gz \cup \Go$ seems a wrong math expression to me. and the lower case $z$ is the vehicle state...} as the zonotope $O$ buffered by the generators of $Z$.
% Then the signed distance \jinsun{you are assuming the reader knows what it is} between $Z$ and $O$ is given by \jinsun{define $\partial$}
% \begin{equation}
%     \sdf(Z, O)  = 
%         \begin{cases}
%           \dist(\cz; \partial \Oz)  & \text{if } Z \cap O =  \emptyset \\
%           -\dist(\cz; \partial  \Oz) & \text{if } Z \cap O \neq \emptyset 
%         \end{cases}, \label{eq:sdf}
% \end{equation}
% where
%     \begin{equation}
%        \dist(\cz; \partial \Oz) = \min_{x \in \partial \Oz} \|\cz - x\|. \label{eq:boundary_distance}
%     \end{equation}
% \end{lem}
% \begin{proof}
% See \cite[Theorem 19]{michaux2023rdf}. 
% \end{proof}

The following theorem leverages the properties of zonotopes to find a closed form expression for the exact signed distance between a collection of zonotopes:
\begin{thm} \label{thm:exact_zono}
Let $\Z = \zonocg{\cz}{\Gz}$ and $\Oj = \zonocg{\coj}{\Goj}$ be zonotopes in $\R^2$ for each $j \in \J$ where $\J$ has a finite number of elements in it.
Let $\Obs = \bigcup_{j \in \J} \Oj$.
Let $\Ojz = \zonocg{\coj}{[\Gz,\Goj]}$.
Suppose that for each $j \in \J$, $\Ojz$ has $N_j$ vertices.
Let $V_j$ be the set of vertices of $\Ojz$ ordered in counterclockwise fashion and $\{h_{i,j}\}_{i=1}^{N_j}$ be the set of line segments between consecutive vertices in $V_j$.

The signed distance between $\Z$ and $\Obs$ is given by 
\begin{align}
   \hspace*{-0.48cm} \sdf(\Z, \Obs)
    % &= \underset{j \in \J}{\min}\: \sdf(Z; \Oj) \nonumber \\
    &=
    \begin{cases}
          \underset{j \in \J}{\min}\: \underset{i \in \{1,\ldots,N_j\} }{\min}\: \dist(\cz; h_{i,j})  & \text{if } \Z \cap \Obs =  \emptyset \\
          -\underset{j \in \J}{\min}\: \underset{i\in \{1,\ldots,N_j\}}{\min}\: \dist(\cz; h_{i,j}) & \text{if } \Z \cap \Obs  \neq \emptyset 
    \end{cases}.  \label{eq:rdf}
\end{align}
% \begin{equation}\label{eq:zonotope_sdf_eq}
%     \sdf(\Z, \mathcal{O}) = 
%         \begin{cases}
%           \underset{i\in \{1,\ldots,N\}}{\min}\: \dist(\cz; h_i)  & \text{if } \Z \cap \mathcal{O} =  \emptyset \\
%           \underset{i\in \{1,\ldots,N\}}{-\min}\: \dist(\cz; h_i) & \text{if } \Z \cap \mathcal{O} \neq \emptyset 
%         \end{cases} .
% \end{equation}
\end{thm}
\begin{proof} 
Assume without loss of generality that $\Z \cap \Oj =  \emptyset$. 
Note that $\sdf(\Z,\Oj) = \dist(\cz; \partial \Ojz)$ because of \cite[Theorem 19]{michaux2023rdf}.
Because $\partial \Ojz = \{ h_{i,j} \}_{i=1}^{N_j}$, the result follows by taking the minimum over $j \in \J$.
The proof for the case $Z \cap \Obs \neq \emptyset$ is similar.
Fig. \ref{fig:zono_sdf} illustrates this proof when the distance is being computed between two zonotopes. 
\end{proof}
Because of Assumptions \ref{ass: offline reachability} and \ref{ass: obs in T}, one can apply Theorem \ref{thm:exact_zono} to compute the constraint in $\opt$. 
However, because \eqref{eq:rdf} still requires computing the distance between a vertex and a finite length line segment, it naively would still require solving a convex quadratic program. 


% In the following theorem, we leverage properties of zonotopes to find a closed form expression for the exact signed distance between two zonotopes:
% \begin{thm} \label{thm:exact_sdf}
% Let $\Z = \zonocg{\cz}{\Gz}$ and $\mathcal{O} = \zonocg{\co}{\Go}$ be zonotopes in $\R^2$ and define $\mathcal{O}_z = \zonocg{c_o}{[\Gz,\Go]}$.
% Suppose $\Oz$ has $N$ vertices, and let $V$ be the set of vertices of $\Oz$ ordered in counterclockwise fashion and $\{h_i\}_{i=1}^N$ be the set of corresponding line segments between consecutive vertices in $V$. 
% Then the signed distance between $\Z$ and $\mathcal{O}$ is
% \begin{equation}\label{eq:zonotope_sdf_eq}
%     \sdf(\Z, \mathcal{O}) = 
%         \begin{cases}
%           \underset{i\in \{1,\ldots,N\}}{\min}\: \dist(\cz; h_i)  & \text{if } \Z \cap \mathcal{O} =  \emptyset \\
%           \underset{i\in \{1,\ldots,N\}}{-\min}\: \dist(\cz; h_i) & \text{if } \Z \cap \mathcal{O} \neq \emptyset 
%         \end{cases} .
% \end{equation}
% \end{thm}
% \begin{proof} 
% Assume without loss of generality that $\Z \cap \mathcal{O} =  \emptyset$. 
% Note that $\sdf(\Z, \mathcal{O}) = \dist(\cz; \partial \Oz)$ because of \cite[Theorem 19]{michaux2023rdf}.
% Because $\partial \Oz = \{ h_i \}_{i=1}^N$, the result follows. 
% % Let $h_i$ be a given line segment comprising the boundary of $\Oz$ and let $\vi{1}$ and $\vi{2}$ be its corresponding ordered vertices. 
% % Then we can parameterize the line containing $h_i$ in terms of $\tau \in \mathbb{R}$ as
% % \begin{equation}
% %     H_i(\tau) = \vi{1} + \tau (\vi{2} - \vi{1})
% % \end{equation}
% % such that $H_i(\tau)$ is on the line segment $h_i$ if $\tau \in [0,1]$. 
% % Then the distance between $c_1$ and $h_i$ can be found by considering  
% % \begin{equation}
% %     \phi_i(\tau) = \|H_i(\tau) - \cz\|_{2} .
% % \end{equation}
% % We can find the minimum of $\phi_i^{2}(\tau)$ and solve for the value $\hat{\tau}_i$ where its gradient vanishes:
% % \begin{equation}
% %     \hat{\tau}_i = \frac{(\cz - \vi{1})^T(\vi{2} - \vi{1})}{(\vi{2} - \vi{1})^T (\vi{2} - \vi{1})}. \label{eq:line_projection}
% % \end{equation}
% % The value $\hat{\tau}_i$ may not be on the line segment $h_i$, so we project it onto the interval $[0,1]$ to get
% % \begin{equation}
% %     \tau^{\ast}_i = \min (\max (\hat{\tau}_i, 0), 1). \label{eq:segment_projection}
% % \end{equation}
% % Then it is clear that $\phi_i(t^{\ast}_i) = \dist(\cz; h_i)$ \jinsun{$\phi_i(\tau^{\ast}_i)$?}.
% % Therefore the distance between $Z$ and $O$ is the minimum distance between $\cz$ and all line segments $h_i$ comprising the boundary of $\Oz$: 
% % \begin{align}
% %     \dist(Z; O) 
% %     &= \dist(\cz; \Oz) \nonumber  \\
% %     &= \underset{i}{\min}\: \phi_i(\tau^{\ast}_i) \nonumber \\ 
% %     &= \underset{i}{\min}\: \dist(\cz; h_i) .  \label{eq:dist}
% % \end{align}
% % % \begin{equation}
% % %     \dist(Z; O) 
% % %     = \dist(\cz; \Oz)
% % %     = \underset{i}{\min}\: \phi_i(\tau^{\ast}_i) 
% % %     = \underset{i}{\min}\: \dist(\cz; h_i) .  \label{eq:dist}
% % % \end{equation}
% The proof for the case $Z \cap \Obs \neq \emptyset$ is similar.
% \end{proof}

% Note that we provide a visual illustration of this theorem in Fig. \ref{fig:zono_sdf}.
% We next show that this result extends to computing the signed distance to a collection of zonotopes.
% \begin{cor}
% Let $\Z = \zonocg{\cz}{\Gz}$ and $\Oj = \zonocg{\coj}{\Goj}$ be zonotopes and define $\Ojz = \zonocg{\coj}{[\Gz,\Goj]}$.
% Denote $\Obs = \underset{j}{\bigcup} \Ojz$.
% Then the signed distance between $Z$ and $\Obs$ is given by 
% \begin{align}
%     \sdf(Z; \Obs) &= \underset{j}{\min}\: \sdf(Z; \Oj) \nonumber \\
%     &=
%     \begin{cases}
%           \underset{j}{\min}\: \underset{i}{\min}\: \dist(\cz; h_{i,j})  & \text{if } Z \cap \Obs =  \emptyset \\
%           -\underset{j}{\min}\: \underset{i}{\min}\: \dist(\cz; h_{i,j}) & \text{if } Z \cap \Obs  \neq \emptyset 
%     \end{cases} ,  \label{eq:rdf}
% \end{align}
% where $\cz$ is the center of $Z$ and $h_{i,j}$ is the $i^{th}$ line segment for $\Ojz$.
% \end{cor}
% \begin{proof}
%     The result follows trivially from Theorem \ref{thm:exact_sdf}.
% \end{proof}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figures/redefine_buffer_obstacle.pdf}
%     \caption{Graphical illustration of signed distance between zonotopes. (Top) The top row illustrates the positive distance function between two zonotopes. First, the gray zonotope is buffered by the generators of the purple zonotope. Then, the distance is computed between the purple zonotope's center and the closest line segment of the buffered zonotope. (Bottom) The bottom row graphically illustrates the negative distance between two zonotopes. First, the pink zonotope's generators buffer the gray zonotope. Then, the negative distance is computed by projecting the pink zonotope's centers on each of the buffered zonotope's half-spaces.} 
%     \label{fig:zono_sdf}
%     \vspace*{-0.2cm}
% \end{figure}

% By using the previous theorem, the next result describes how to compute the distance between the ego vehicle and obstacles.\jon{reword?}
% \begin{thm} \label{thm:exact_rdf}
%     Suppose the ego vehicle is starting from initial condition $z_0\in\Z_0$ with control parameter $p\in\PP$.
%     Let $\xi$ and $\vartheta$ be the zonotope reachable set and zonotope obstacle representation as in Assumptions \ref{ass: offline reachability} and \ref{ass: obs in T}, respectively. 
%     Then $\rdf(\xi(z_0,p), \vartheta(k)) \leq \rdf( \{\E\big(t,z_0,p\big)\}_{t\in T}, \{\Obskt\}_{t \in T})$. 
% \end{thm}
% \begin{proof}We prove the desired result by considering two cases. 
% First assume  $\FOt \cap \Obst  = \emptyset$ for all $t \in T$ and let $\FOT = \{\E\big(t,z_0,p\big)\}_{t\in T}$ and $\ObskT = \{\Obskt\}_{t \in T}$.
% Then
% \begin{align}
%     \rdf(\FOT, \ObskT) &= \min_{t \in T} \sdf(\FO\big(t,z_0,p\big), \Obskt) \\
%     &\geq \underset{j \in \J}{\min}\: \sdf(\FOzj \big(z_0,p\big), \vartheta(j,k)) \\
%     &= \underset{j \in \J}{\min}\: \underset{i\in \{1,\ldots,N_j\}}{\min}\: \dist(\cj; h_{i,j}) \\
%     &= \underset{j \in \J}{\min}\: \rdf(\xi(z_0,p), \vartheta(j,k)) \\
%     &= \ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj)
% \end{align}
% where the first equality follows from the definition of $\rdf$ in Def. \ref{def:rdf_point}, the second inequality follows from Assumption \ref{ass: offline reachability}, the third equality follows from Theorem \ref{thm:exact_sdf}, the fourth \stkout{inequality} \new{equality} by flipping the order of minimization. 
% Thus $\ardf$ underapproximates the positive distance between the forward occupancy and an obstacle. 

% If instead $\FOt \cap \Obst \neq \emptyset$ for some $t \in T$, replacing $\geq$ with $\leq$ shows that $\ardf$ overrapproximates the negative distance between an obstacle and the forward occupancy.
% \jon{should the negative distance be an underapproximation too?} \jinsun{I think it is an overapproximation in the negative case}
% \end{proof}
% \begin{thm} \label{thm:exact_rdf}
%     Suppose the ego vehicle is starting from initial condition $z_0\in\Z_0$ with control parameter $p\in\PP$.
%     Consider an obstacle $\Obst$ with a zonotope representation.
%     Let $\{\FOzj\}$ \jinsun{mention Assumption 7 here?} be the zonotope reachable set overapproximating the ego vehicle's trajectory.
%     Define $\ardf_j$ as the following: \jon{reword}
%     \begin{equation}
%     \label{eq:ardf_j}
%     \ardf_j(\FOzj; \Obszj) = 
%         \begin{cases}
%           \underset{i}{\min}\: \dist(\cz; h_{i,j})  & \text{if } \FOzj \cap \Obszj  =  \emptyset \\
%           -\underset{i}{\min}\: \dist(\cz; h_{i,j})  & \text{if } \FOzj \cap \Obszj  \neq  \emptyset,
%         \end{cases} 
%     \end{equation}
%     \jinsun{$\Obszj$? conflict with Defintion 5}
%     where $\cj$ \jinsun{where is it used?} is the center of zonotope $\FOzj$, and $h_{i,j}$ is the $i^{th}$ line segment of the obstacle zonotope buffered by the generators of $\FOzj$.
%     Now define the function $\ardf$ as:
%     \begin{equation}
%     \label{eq:ardf}
%         \ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj) = \underset{j \in \J}{\min}\ardf_j(\FOzj; \Obszj).
%     \end{equation}
% If $\FOT \cap \ObsT = \emptyset$, then $\ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj) \leq \rdf(\FOT; \ObsT)$.
% If $\FOT \cap \ObsT \neq \emptyset$, then $\ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj) \geq \rdf(\FOT; \ObsT)$.
% \end{thm}
% \begin{proof}We prove the desired result by considering two cases. 
% First assume  $\FOt \cap \Obst  = \emptyset$ for all $t \in T$. 
% Then
% \begin{align}
%     \rdf(\FOT; \ObsT) &= \min_{t \in [0, \tf]} \sdf(\FO\big(t,z_0,p\big); \Obst) \\
%     &\geq \underset{j \in \J}{\min}\: \sdf(\FOzj \big(z_0,p\big); \Obszj) \\
%     &= \underset{j \in \J}{\min}\: \underset{i \in \I}{\min}\: \dist(\cj; h_{i,j}) \\
%     &= \underset{j \in \J}{\min}\: \ardf_j(\FOzj; \Obszj) \\
%     &= \ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj)
% \end{align}
% where the first equality follows from the definition of $\rdf$ in Def. \ref{def:rdf_point}, the second inequality follows from Assumption \ref{ass: offline reachability}, the third equality follows from Theorem \ref{thm:exact_sdf}, the fourth \stkout{inequality} \new{equality} by flipping the order of minimization. 
% Thus $\ardf$ underapproximates the positive distance between the forward occupancy and an obstacle. 

% If instead $\FOt \cap \Obst \neq \emptyset$ for some $t \in T$, replacing $\geq$ with $\leq$ shows that $\ardf$ overrapproximates the negative distance between an obstacle and the forward occupancy.
% \jon{should the negative distance be an underapproximation too?} \jinsun{I think it is an overapproximation in the negative case}
% \end{proof}


% For this result to be useful, we need to extend it to multiple zonotopes, which we do next:



% \subsection{Main Theorem}
% \jon{Is this the main theorem?}
% In this subsection we introduce the main theorem used to compute the exact distance between approximation to the reachability-based distance function.
% \stkout{In this section w}\new{W}e derive an approximation to the true RDF using zonotope arithmetic.
% We start by defining a distance function between  \jinsun{unfinished sentence}
% \begin{defn}\label{def:rdf_point}
% Given initial condition $z_0\in\Z_0$ and control parameter $p\in\PP$, the \defemph{reachability-based distance} function associated with the forward occupancy \stkout{$\FOt$} \new{$\E\big(t,z_0,p\big)$} \jinsun{it contradicts with the definition of $\E$ in \eqref{eq: def occupancy}} \challen{Fixed} of the ego vehicle and obstacle $\Obst$ \jinsun{So obstacles are no longer indexed?} over the interval $T = [0, \tf]$ is a mapping defined by
% \begin{equation}
%     \rdf(\FOT; \ObsT) = \min_{t \in [0, \tf]} \sdf(\FO\big(t,z_0,p\big); \Obst).
% \end{equation}
% \jinsun{$\FOT$ is improper because by definition $\E$ cannot take an interval as its argin}
% \jon{why not?}
% \end{defn}
% By using zonotopes, the next theorem approximates the distance between the ego vehicle and obstacles.\jon{reword}

% \begin{thm} \label{thm:exact_rdf}
%     Suppose the ego vehicle is starting from initial condition $z_0\in\Z_0$ with control parameter $p\in\PP$ and satisfies \eqref{eq: dyn tilde_z} for all $t \in [0, \tf]$.
%     Consider an obstacle $\Obst$ with a zonotope representation.
%     Let $\{\FOzj\}$ \jinsun{mention Assumption 7 here?} be the zonotope reachable set overapproximating the ego vehicle's trajectory.
%     Define $\ardf_j$ as the following: \jon{reword}
%     \begin{equation}
%     \label{eq:ardf_j}
%     \ardf_j(\FOzj; \Obszj) = 
%         \begin{cases}
%           \underset{i}{\min}\: \dist(\cz; h_{i,j})  & \text{if } \FOzj \cap \Obszj  =  \emptyset \\
%           -\underset{i}{\min}\: \dist(\cz; h_{i,j})  & \text{if } \FOzj \cap \Obszj  \neq  \emptyset,
%         \end{cases} 
%     \end{equation}
%     \jinsun{$\Obszj$? conflict with Defintion 5}
%     where $\cj$ \jinsun{where is it used?} is the center of zonotope $\FOzj$, and $h_{i,j}$ is the $i^{th}$ line segment of the obstacle zonotope buffered by the generators of $\FOzj$.
%     Now define the function $\ardf$ as:
%     \begin{equation}
%     \label{eq:ardf}
%         \ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj) = \underset{j \in \J}{\min}\ardf_j(\FOzj; \Obszj).
%     \end{equation}
% If $\FOT \cap \ObsT = \emptyset$, then $\ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj) \leq \rdf(\FOT; \ObsT)$.
% If $\FOT \cap \ObsT \neq \emptyset$, then $\ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj) \geq \rdf(\FOT; \ObsT)$.
% \end{thm}
% \begin{proof}We prove the desired result by considering two cases. 
% First assume  $\FOt \cap \Obst  = \emptyset$ for all $t \in T$. 
% Then
% \begin{align}
%     \rdf(\FOT; \ObsT) &= \min_{t \in [0, \tf]} \sdf(\FO\big(t,z_0,p\big); \Obst) \\
%     &\geq \underset{j \in \J}{\min}\: \sdf(\FOzj \big(z_0,p\big); \Obszj) \\
%     &= \underset{j \in \J}{\min}\: \underset{i \in \I}{\min}\: \dist(\cj; h_{i,j}) \\
%     &= \underset{j \in \J}{\min}\: \ardf_j(\FOzj; \Obszj) \\
%     &= \ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj)
% \end{align}
% where the first equality follows from the definition of $\rdf$ in Def. \ref{def:rdf_point}, the second inequality follows from Assumption \ref{ass: offline reachability}, the third equality follows from Theorem \ref{thm:exact_sdf}, the fourth \stkout{inequality} \new{equality} by flipping the order of minimization. 
% Thus $\ardf$ underapproximates the positive distance between the forward occupancy and an obstacle. 

% If instead $\FOt \cap \Obst \neq \emptyset$ for some $t \in T$, replacing $\geq$ with $\leq$ shows that $\ardf$ overrapproximates the negative distance between an obstacle and the forward occupancy.
% \jon{should the negative distance be an underapproximation too?} \jinsun{I think it is an overapproximation in the negative case}
% \end{proof}

\subsection{Neural Network Architecture}
\label{subsec:nn_architecture}
We now use results from Section \ref{subsec:rdf_derivation} to enable the closed form expression of the signed distance function between zonotopes.
In particular, we show that the signed distance between collections of zonotopes can be computed exactly with an implicit neural network with fixed, prespecified weights.
% We then generalize the network to compute the signed distance to a collection of zonotopes.
% between the forward occupancy of the ego vehicle and obstacles in the environment
Before constructing this network, we note the following observation about max and min operations which was proven in \cite[Lemma D.3]{arora2016} \cite[Section 3.2]{ferlez2020}:

\begin{lem}\label{lem:minmax}
% Let $W ^{\min}, b ^{\min},W ^{\max},$ and $b ^{\max}$ be defined as:
% % The functions $\min(x,y)$ and $\max(x,y)$ can be specified as ReLU networks with weights $\Theta^{\min} = (W ^{\min}, b ^{\min})$ and $\Theta^{\max} = (W ^{\max}, b ^{\max})$ such that
% \begin{align}
%     W ^{\min} &= 
%     \begin{bmatrix}
%             1 & 1 \\
%             1 & -1 \\
%             -1 & 1 \\
%             -1 & -1
%     \end{bmatrix},
%     b^{\min} = 
%     \begin{bmatrix}
%         \frac{1}{2} & -\frac{1}{2} & -\frac{1}{2} & -\frac{1}{2}
%     \end{bmatrix}
% \end{align}
% \begin{align}
%     W^{\max} &= 
%     \begin{bmatrix}
%             1 & 1 \\
%             -1 & -1 \\
%             -1 & 1 \\
%             1 & -1
%     \end{bmatrix},
%      b^{\max} =
%     \begin{bmatrix}
%         \frac{1}{2} & -\frac{1}{2} & \frac{1}{2} & \frac{1}{2}
%     \end{bmatrix}.
% \end{align}
The maximum or minimum of a pair of numbers can be computed using a ReLU network with width of $4$ and a depth of $2$ as:
\begin{align}
\min(x,y) &= \relu \left(   \begin{bmatrix}
            1 & 1 \\
            1 & -1 \\
            -1 & 1 \\
            -1 & -1
    \end{bmatrix} \begin{bmatrix} x \\ y \end{bmatrix} \right)^T  \begin{bmatrix}
        \frac{1}{2} \\ -\frac{1}{2} \\ -\frac{1}{2} \\ -\frac{1}{2}
    \end{bmatrix} \\ 
\max(x,y) &= \relu \left(  \begin{bmatrix}
            1 & 1 \\
            -1 & -1 \\
            -1 & 1 \\
            1 & -1
    \end{bmatrix} \begin{bmatrix} x \\ y \end{bmatrix} \right)^T\begin{bmatrix}
        \frac{1}{2} \\ -\frac{1}{2} \\ \frac{1}{2} \\ \frac{1}{2}
    \end{bmatrix}.
\end{align}
\end{lem}

% \begin{lem}\label{lem:minmax}
% Let $W ^{\min}, b ^{\min},W ^{\max},$ and $b ^{\max}$ be defined as:
% % The functions $\min(x,y)$ and $\max(x,y)$ can be specified as ReLU networks with weights $\Theta^{\min} = (W ^{\min}, b ^{\min})$ and $\Theta^{\max} = (W ^{\max}, b ^{\max})$ such that
% \begin{align}
%     W ^{\min} &= 
%     \begin{bmatrix}
%             1 & 1 \\
%             1 & -1 \\
%             -1 & 1 \\
%             -1 & -1
%     \end{bmatrix},
%     b^{\min} = 
%     \begin{bmatrix}
%         \frac{1}{2} & -\frac{1}{2} & -\frac{1}{2} & -\frac{1}{2}
%     \end{bmatrix}
% \end{align}
% \begin{align}
%     W^{\max} &= 
%     \begin{bmatrix}
%             1 & 1 \\
%             -1 & -1 \\
%             -1 & 1 \\
%             1 & -1
%     \end{bmatrix},
%      b^{\max} =
%     \begin{bmatrix}
%         \frac{1}{2} & -\frac{1}{2} & \frac{1}{2} & \frac{1}{2}
%     \end{bmatrix}.
% \end{align}
% The maximum or minimum of a pair of numbers can be computed using a ReLU network with width of $4$ and a depth of $2$ as:
% \begin{align}
% \min(x,y) &= \relu \left(  W ^{\min} \begin{bmatrix} x \\ y \end{bmatrix} \right)^T b^{\min} \\ 
% \max(x,y) &= \relu \left(  W ^{\max} \begin{bmatrix} x \\ y \end{bmatrix} \right)^T b^{\max}.
% \end{align}
% \end{lem}
% \begin{proof}
%     See Lem. D.3 of \cite{arora2016} and Sec. 3.2 of \cite{ferlez2020}.
% \end{proof}


% \begin{lem}\label{lem:minmax}
% The functions $\min(x,y)$ and $\max(x,y)$ can be specified as ReLU networks with weights $\Theta^{\min} = (W ^{\min}, b ^{\min})$ and $\Theta^{\max} = (W ^{\max}, b ^{\max})$ such that
% \begin{align}
%     W ^{\min} &= 
%     \begin{bmatrix}
%             1 & 1 \\
%             1 & -1 \\
%             -1 & 1 \\
%             -1 & -1
%     \end{bmatrix},
%     b^{\min} = 
%     \begin{bmatrix}
%         \frac{1}{2} & -\frac{1}{2} & -\frac{1}{2} & -\frac{1}{2}
%     \end{bmatrix}
% \end{align}
% and 
% \begin{align}
%     W^{\max} &= 
%     \begin{bmatrix}
%             1 & 1 \\
%             -1 & -1 \\
%             -1 & 1 \\
%             1 & -1
%     \end{bmatrix},
%      b^{\max} =
%     \begin{bmatrix}
%         \frac{1}{2} & -\frac{1}{2} & \frac{1}{2} & \frac{1}{2}
%     \end{bmatrix}.
% \end{align}
% \end{lem}
% \begin{proof}
%     See Lem. D.3 of \cite{arora2016} and Sec. 3.2 of \cite{ferlez2020}.
% \end{proof}
By applying Lemma \ref{lem:minmax} recursively, one can implement multi-element min(max) operations with ReLU networks and construct the following bound:
% It is straightforward to generalize Lem. \ref{lem:minmax} to implement multi-element min(max) operations with ReLU networks \cite{arora2016, ferlez2020}.
\begin{cor}
\label{cor:relu_minmax_size}
The minimum (maximum) of $N$ numbers can be represented exactly with a ReLU network with width and depth bounded by $4 \cdot \bigl \lceil \frac{N}{2} \bigr \rceil$ and $2 \cdot \lfloor \log_{2} N \rfloor $, respectively.
\end{cor}
% \begin{proof}
%     See Lem. D.3 of \cite{arora2016} and Sec. 3.2 of \cite{ferlez2020}.
% \end{proof}
One can apply these results to prove the following theorem:
\begin{thm}
\label{thm:relu_sdf_network}
Let $\Z = \zonocg{\cz}{\Gz}$ and $\Oj = \zonocg{\coj}{\Goj}$ be zonotopes in $\R^2$ for each $j \in \J$ where $\J$ has a finite number of elements in it.
Let $\Obs = \bigcup_{j \in \J} \Oj$.
Let $\Ojz = \zonocg{\coj}{[\Gz,\Goj]}$.
Suppose that for each $j \in \J$, $\Ojz$ has $N_j$ vertices.
Then the signed distance between $\Z$ and $\Obs$ can be represented \textbf{exactly} using a ReLU network
width and depth bounded by  $4 \cdot \bigl \lceil \sum_{j \in \J} \frac{\sum_{j \in \J} N_j }{2} \bigr \rceil + 8$ and $2 \cdot \lfloor \log_{2}  ( \sum_{j \in \J} N_j ) \rfloor + 4$, respectively.
% with $2 \sum_{ j \in \J} N_j$ ReLU operations. 
% The signed distance between a collection of zonotopes can be represented \textbf{exactly} using a ReLU network.
\end{thm}
\begin{proof} 
Let $V_j$ be the set of vertices of $\Ojz$ ordered in counterclockwise fashion and $\{h_{i,j}\}_{i=1}^{N_j}$ be the set of line segments between consecutive vertices in $V_j$.
Using Theorem \ref{thm:exact_rdf}, one can compute the signed distance between $\Z$ and $\Obs$ by applying Lemma \ref{lem:minmax}, if one can compute $\dist(\cz; h_{i,j})$.

Let $v_{i,j}$ and $v_{i+1,j}$ be the vertices corresponding to line segment $h_{i,j}$.   
Let $H_{i,j}(\tau) = v_{i,j} + (v_{i+1,j} - v_{i,j})\tau$, which is the line that extends $h_{i,j}$.

The projection of $\cz$ onto $H_{i,j}$ is
\begin{equation}
    \hat{t}_{i,j} = \frac{(\cz - v_{i,j})^T(v_{i+1,j} - v_{i,j})}{(v_{i+1,j} - v_{i,j})^T (v_{i+1,j} - v_{i,j})}.
\end{equation}
Note that $H_{i,j}(\hat{t}_{i,j})$ is the point on $H_{i,j}$ closest to $\cz$, but it may not be on the line segment $h_i$.
Therefore it is necessary to project $\hat{t}_{i,j}$ onto the interval $[0,1]$:
\begin{equation}\label{eq:segment_projection}
     t_{i,j}^{\ast} = \min (\max (\hat{t}_{i,j}, 0), 1).
\end{equation}
One can compute \eqref{eq:segment_projection} using Lemma \ref{lem:minmax} by performing $2$ ReLU operations, which requires a ReLU network of width and depth bounded by $8$ and $4$, respectively. 
Then the distance between $\cz$ and $h_i$ is 
\begin{equation}\label{eq:segment_distance}
    \dist(\cz; h_i) = \| \cz - (v_i + (v_{i+1} - v_i)t_i^{\ast})\|_{2}.
\end{equation}

The result follows by noting that to compute the signed distance between $\Z$ and $\Obs$ using \eqref{eq:rdf}, one needs to perform \eqref{eq:segment_projection} once for each line segment in $\Ojz$ and noting that $\Obs$ has $\sum_{j\in \J} N_j$ line segments.
\end{proof}

% \begin{thm}
% \label{thm:relu_sdf_network}
% Let $\Z = \zonocg{\cz}{\Gz}$ and $\Oj = \zonocg{\coj}{\Goj}$ be zonotopes in $\R^2$ for each $j \in \J$ where $\J$ has a finite number of elements in it.
% Let $\Obs = \bigcup_{j \in \J} \Oj$.
% Let $\Ojz = \zonocg{\coj}{[\Gz,\Goj]}$.
% Suppose that for each $j \in \J$, $\Ojz$ has $N_j$ vertices.
% Then the signed distance between $\Z$ and $\Obs$ can be represented \textbf{exactly} using a ReLU network with $2 \sum_{ j \in \J} N_j$ ReLU operations. 
% % The signed distance between a collection of zonotopes can be represented \textbf{exactly} using a ReLU network.
% \end{thm}
% \begin{proof} 
% Let $V_j$ be the set of vertices of $\Ojz$ ordered in counterclockwise fashion and $\{h_{i,j}\}_{i=1}^{N_j}$ be the set of line segments between consecutive vertices in $V_j$.
% Let $v_{i,j}$ and $v_{i+1,j}$ be the vertices corresponding to line segment $h_i$.   
% As a result of Theorem \ref{thm:exact_rdf}, one can compute the signed distance between $\Z$ and $\Obs$ by applying Lemma \ref{lem:minmax}, if one can compute $\dist(\cz; h_{i,j})$.

% Let $H_{i,j}(\tau) = v_{i,j} + (v_{i+1,j} - v_{i,j})\tau$, which is the line that extends $h_{i,j}$.
% Then the projection of $\cz$ onto $H_{i,j}$ is
% \begin{equation}
%     \hat{t}_{i,j} = \frac{(\cz - v_{i,j})^T(v_{i+1,j} - v_{i,j})}{(v_{i+1,j} - v_{i,j})^T (v_{i+1,j} - v_{i,j})}.
% \end{equation}
% Note that $H_{i,j}(\hat{t}_{i,j})$ is the point on $H_{i,j}$ closest to $\cz$, but it may not be on the line segment $h_i$.
% Therefore it is necessary to project $\hat{t}_{i,j}$ onto the interval $[0,1]$:
% \begin{equation}\label{eq:segment_projection}
%      t_{i,j}^{\ast} = \min (\max (\hat{t}_{i,j}, 0), 1).
% \end{equation}
% One can compute \eqref{eq:segment_projection} using Lemma \ref{lem:minmax} by performing $2$ ReLU operations. 

% can be computed using Lemma  \ref{lem:minmax}. 
% By Lem. \ref{lem:minmax}, eq \eqref{eq:segment_projection} can be computed with ReLU networks with weights $\Theta^{\min} = (W ^{\min}, b ^{\min})$ and $\Theta^{\max} = (W ^{\max}, b ^{\max})$
% \begin{align}
%     \Tilde{t}_i &= \mathbf{relu}(W^{\max} \cdot \begin{bmatrix}\hat{t}_i \\ 0\end{bmatrix})^T b^{\max}  \\
%     t_i^{\ast} &= \mathbf{relu}(W^{\min} \cdot \begin{bmatrix}\Tilde{t}_i \\ 1\end{bmatrix})^T b^{\min}.
% \end{align}
% Then the distance between $\cz$ and $h_i$ is
% \begin{equation}\label{eq:segment_distance}
%     \dist(\cz; h_i) = \| \cz - (v_i + (v_{i+1} - v_i)t_i^{\ast})\|_{2}.
% \end{equation}
% We then obtain the signed distance between $\Z$ and $\mathcal{O}$ from Thm. \ref{thm:exact_zono} by computing $\underset{i\in \{1,\ldots,N\}}{\min}\: \dist(\cz; h_i)$ with a ReLU network with width and depth bounds given by Cor. \ref{cor:relu_minmax_size}.
% \end{proof}

% \begin{rem}
%     This result can be trivially extended to compute the signed distance to a collection of $M$ zonotopes by batching the computations described in Thm \ref{thm:relu_sdf_network} and passing the output to another ReLU network that computes the minimum of $M$ numbers.
% \end{rem}


\subsection{Trajectory Optimization}


\subsection{Online Operation}


==> sections/old/07_rdf.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%~~~~~~~~~~~~~~~~~~~~~~~Overview of RDFs
\section{Reachability-based Signed Distance Functions}
\label{sec:RDF}
\jon{We can either 1) place this in the prelim section; 2) combine with Neural net section; 3) remove altogether}
% This section defines the signed distance function between sets. 
% Signed distance functions are used in robotics in a variety of applications including representing collision avoidance constraints. 
This section describes how to extend the signed distance function to a distance function between the forward reachable set of a robot and an obstacle. 
This novel distance function, which we call the reachability-based signed distance function (\methodname{}), was introduced in \cite{michaux2023rdf} and  enables us to formulate the collision avoidance problem between a parameterized reachable set and an obstacle as an optimization problem. 

\subsection{Signed Distance Functions}
We begin by defining an unsigned distance function:
\begin{defn}
Given a set $\Omega \subset \mathbb{R}^{\nd}$, the \defemph{distance function} associated with $\Omega$ is defined by
    \begin{equation}
       \dist(x;\Omega) = \min_{y \in \partial\Omega} \|x - y\|.
    \end{equation}
The \defemph{distance between two sets} $\Omega_1, \Omega_2 \subset \mathbb{R}^{\nd}$ is defined by
    \begin{equation}
       \dist(\Omega_1,\Omega_2) = \min_{\substack{x \in \partial\Omega_1 \\ y \in \partial\Omega_2}} \|x - y\|.
    \end{equation}
\end{defn}
\textbf{Notice that this distance function is zero for sets that have non-trivial intersection. 
As a result, this distance function provides limited information for such sets (i.e., it is unclear how much they are intersecting with one another).
To address this limitation, we consider the following definition:}
\begin{defn} Given a subset $\Omega$ of $\mathbb{R}^{\nd}$, the \defemph{signed distance function} $\sdf$ between a point is a map $\sdf: \mathbb{R}^{\nd} \to \mathbb{R}$ defined as
    \begin{equation}
    \sdf(x; \Omega) = 
        \begin{cases}
          \dist(x, \partial\Omega)  & \text{if } x \not \in \Omega \\
          -\dist(x,\partial\Omega) & \text{if } x \in \Omega.
        \end{cases}
\end{equation}
The \defemph{signed distance between two sets} $\Omega_1, \Omega_2 \subset \mathbb{R}^{\nd}$ is defined as
    \begin{equation}
    \sdf(\Omega_1,\Omega_2) = 
        \begin{cases}
          \dist(\Omega_1,\Omega_2)  & \text{if } \Omega_1 \cap \Omega_2 = \emptyset  \\
          -\dist(\Omega_1,\Omega_2) & \text{otherwise}.
        \end{cases}
\end{equation}
\end{defn}
% \begin{itemize}
%     \item Signed distance functions are a common representation in robotics.
%     \item In this section we give a brief overview of signed distance functions and describe some of their notable properties.
%     \item In the context of motion planning the SDF has been used to compute the distance between a single configuration of a robot and a static obstacle \cite{XXX}.
%     \item We then introduce the reachability-based distance function, which represents the distance to a swept volume.
% \end{itemize}


\subsection{Reachability-Based Signed Distance Functions}
This subsection describes the reachability-based distance function as the signed distance function associated with the forward reachable set of the ego vehicle.
% The following sections describe how to overapproximate the forward occupancy and distance calculations with zonotopes using reachability analysis.
\begin{defn}\label{def:rdf_point}
The \defemph{reachability-based distance} function associated with the forward occupancy reachable set $\FO$ is a mapping 
defined by
\begin{equation}
    \rdf(x, \FO) = \min_{j \in \Nj} \rdf_j(x;\FO_j)
\end{equation}
where
$\rdf_j$ is the signed distance function associated with the $j^{th}$ forward occupancy $\FO_j$ such that
\begin{equation}
    \rdf_j(x;\FO_j) = \sdf(x;\FO_j).
\end{equation}
The \defemph{reachability-based distance} between an obstacle $O \subset \mathbb{R}^d$ and the robot's forward occupancy reachable set $\FO$ is defined by
\begin{equation}
    \rdf(O, \FO) = \min_{j \in \Nj} \rdf_j(O, \FO_j).
\end{equation}
\end{defn}
One can use this distance function to formulate trajectory optimization problems as we describe next. \jon{This statement is out of place}



==> sections/overview.tex <==
\section{Robot Representation}
\jon{Add this stuff from the appendix and reorg. We provide a brief overview of the arm representation.}
% Note that $B_p(c,r)$ refers to an $L_p$ ball in $\mathbb{R}^3$ centered at $c$ with radius $r$.

\subsection{Arm Kinematics}
\label{app:modeling_arm_kinematics}
\jon{Condense this section}
Given a compact time interval $T \subset \R$, we define a trajectory for the robot's configuration as $q: T \to Q \subset \R^{\nq}$ and a trajectory for the velocity as $\dot{q}: T \to \R^{\nq}$.
We restate an assumption \cite[Ass. 4]{michaux2024sparrows} about the robot model:
\begin{assum}\label{assum:robot}
The robot operates in an three-dimensional workspace, denoted $\workspace \subset \R^{3}$, such that $\workspace \subset \world$.
There exists a reference frame called the base frame, denoted the $0$\ts{th} frame, that indicates the origin of the robot's kinematic chain.
We assume the robot's base frame coincides with the origin of the world frame.
The robot is fully actuated and composed of only revolute joints, where the $j$\ts{th} joint actuates the robot's $j$\ts{th} link.
The robot's $j$\ts{th} joint has position and velocity limits given by $\qj \in [\qlim^-, \qlim^+]$ and $\qdj \in [\dqlim^-, \dqlim^+]$ for all $t \in T$, respectively. 
The robot's input is given by $u: T \to \R^{\nq}$.
\end{assum}
% Recall from Assum. \ref{assum:robot} that the transformation from \textit{world} from to the the robot's $0$\ts{th}, or \textit{base}, frame is known.
% We further assume that the robot's $j$\ts{th} reference frame $\{\hat{x}_j, \hat{y}_j, \hat{z}_j\}$ is attached to the robot's $j$\ts{th} revolute joint, and that $\hat{z}_j = [0, 0, 1]^\top$ corresponds to the $j$\ts{th} joint's axis of rotation.
We also assume that the robot's $j$\ts{th} reference frame $\{\hat{x}_j, \hat{y}_j, \hat{z}_j\}$ is attached to the robot's $j$\ts{th} revolute joint, and that $\hat{z}_j = [0, 0, 1]^\top$ points in direction of the $j$\ts{th} joint's axis of rotation.
Then $\FK_j: Q \to \R^{4 \times 4}$ maps the robot's time-dependent configuration to the pose of the $j$\ts{th} joint in the world frame:
\begin{equation}
\label{eq:fk_j}
    \FK_j(\q) = 
    \begin{bmatrix} R_j(\q) & p_j(\q) \\
    \zeros  & 1 \\
    \end{bmatrix},
\end{equation}
where 
\begin{equation}\label{eq:fk_pos_j}
    p_j(\q) = \sum_{l=1}^{j} R_{l}(\q) p_{l}^{l-1}.
\end{equation}
and 
\begin{equation}\label{eq:fk_orn_j}
    R_j(\q) \coloneqq R_j^{0}(\q) = \prod_{l=1}^{j}R_{l}^{l-1}(\ql)
\end{equation}
are the position and orientation of frame $j$ with respect to world frame $\world$, respectively.

For simplicity, Assum. \ref{assum:robot} only specifies revolute joints to simplify the description of the forward kinematics; the methods described in this paper readily extend to other joint types.
We also ignore any uncertainty in the robot's dynamics, and instead assume that one could apply an inverse dynamics controller \cite{spong2005textbook}  to track any trajectory of the robot perfectly.
As a result, this work focuses exclusively on modeling the kinematic behavior of the robotic arm.

\subsection{Arm Occupancy}
\label{app:modeling_arm_occupancy}
\jon{reorganize this section}
In this subsection, we define the \textit{forward occupancy} as the volume occupied by the arm in the workspace $\workspace$.
% We next use the arm's forward kinematics \eqref{eq:fk_j} to define the \textit{forward occupancy} which is the volume occupied by the arm in the workspace $\workspace$.
Let $L_j \subset \workspace \subset \R^3$ denote the volume occupied by the robot's $j$\ts{th} link with respect to the $j$\ts{th} reference frame. 
Then the forward occupancy of link $j$ is the map $\FO_j: Q \to \pow{\workspace}$ defined as
\begin{align}\label{eq:link_occupancy}
     \FO_j(\q) &= p_j(\q) \oplus R_j(\q) L_j,
\end{align}
where $p_j(\q)$ and $R_j(\q)$ specify the pose of the $j$\ts{th} joint, and $R_j(\q) L_j$ is the rotated volume of link $j$.
The volume occupied by the entire arm in the workspace is then defined by the map $\FO: Q \to \workspace$ such that
\begin{align}\label{eq:forward_occupancy}
    \FO(\q) = \bigcup_{j = 1}^{\nq} \FO_j(\q) \subset \workspace. 
\end{align}
Because the geometry of any of the robot's links may be arbitrarily complex, we restate an assumption \cite[Ass. 5]{michaux2024sparrows} that simplifies the construction of an overapproximation to the forward occupancy:
\begin{assum}\label{assum:joint_link_occupancy}
    Given a robot configuration $\q$ and any $j \in \{1,\dots, \nq\}$, there exists a ball with center $p_j(\q)$ and radius $r_j$  that overapproximates the volume occupied by the $j$\ts{th} joint in $\workspace$.
    We further assume that link volume $L_j$ is a subset of the tapered capsule formed by the convex hull of the balls overapproximating the $j$\ts{th} and $j+1$\ts{th} joints.
    % See Fig. \ref{fig:assumption_figure}.
\end{assum}

Following Assum. \ref{assum:joint_link_occupancy}, we now define the ball $\Sjq$ overapproximating the volume occupied by the $j$\ts{th} joint as 
\begin{equation}\label{eq:joint_occupancy}
    \Sjq = \Btwo(p_j(\q), r_j)
\end{equation}
and the tapered capsule $TC_j(q(t))$ overapproximating the $j$\ts{th} link as
\begin{equation}
 TC_j(q(t)) = \conv\Big( \Sjq \cup \Sjpq \Big).
\end{equation}
Then, the volumes occupied by the $j$\ts{th} link \eqref{eq:link_occupancy} and the entire arm \eqref{eq:forward_occupancy} can be overapproximated by
% \begin{align}\label{eq:link_capsule_occupancy}
%      \FO_j(\q)  &\subset \conv\Big( \Sjq \cup \Sjpq \Big) = TC_j(q(t)) \\
%      &= TC_j(q(t)),
% \end{align}
\begin{equation}\label{eq:link_capsule_occupancy}
     % \FO_j(\q)  \subset \conv\Big( \Sjq \cup \Sjpq \Big) = TC_j(q(t))
     \FO_j(\q)  \subset TC_j(q(t))
\end{equation}
and
\begin{equation} \label{eq:forward_capsule_occupancy}
    \FO(\q) \subset \bigcup_{j = 1}^{\nq} TC_j(q(t)) \subset \workspace, 
\end{equation}
respectively.

For convenience, the notation $\FO(q(T))$ denotes the forward occupancy over an entire time interval $T$.
$\FO(q(T))$ is also called the \emph{reachable set} of the robot.
Notably, the arm is \emph{collision-free} over the time interval $T$ if $\FO(q(T))$ does not intersect with the environment.


To facilitate the exposition of our approach, we summarize the construction of the robot's safety representation in the following theorem:
% \begin{assum}\label{assum:splanning}
% We assume the robot is a serial manipulator with $n_q \in \N$ revolute joints.
% We assume that the swept volume (i.e. reachable set) corresponding to the robot's motion is overapproximated by a collection of $L_2$ balls in $\R^3$, which we call the \SFO ($\sfo$) \cite{michaux2024sparrows}.
% The $\sfo$ is composed of closed balls of the form
% \begin{equation}
%     \Sbarjimk = \Btwo\left(\bar{c}_{j,i,m}(k), \bar{r}_{j,i,m}(k)\right),
% \end{equation}
% where $k \in K$ parameterizes the robot's trajectories, $\pz{T_i}$ is an overapproximation of the $i$\ts{th} time interval, and $\pzqjki$ is an overapproximation of the robot's $j$\ts{th} joint position, and $m \in N_S = \{1,\dots, n_S\}$ indexes the balls along each of the robot's links.
% \end{assum}
\begin{thm}\label{thm:sparrows}
% We assume the robot is a serial manipulator with $n_q \in \N$ revolute joints.
% We assume that there exists a partition of $T$ using a finite set of intervals, $T_i$ (i.e., $T = \cup_{i=1}^{n_t} T_i$).
% Then the swept volume (i.e., reachable set) corresponding to the robot's motion is overapproximated by a collection of $L_2$ balls in $\R^3$, which we call the \SFO ($\sfo$) \cite{michaux2024sparrows}.
% Formally, the $\sfo$ is defined as 
Given a serial manipulator with $n_q \in \N$ revolute joints, a time partition $T$ of a finite set of intervals, $T_i$ (i.e., $T = \cup_{i=1}^{n_t} T_i$), the swept volume corresponding to the robot's motion over $T$ is overapproximated by a collection of $L_2$ balls in $\R^3$, which we call the \SFO ($\sfo$) \cite{michaux2024sparrows} defined as \jon{make sure notation matches the appendix.}
\begin{equation}\label{eq:simple_sfo}
\sfo = \cup_{j=1}^{n_q} \cup_{i=1}^{n_t} \cup_{m=1}^{n_S} S_{j,i,m}(q_j(T_i; k)),
% = B\left(c_{j,i,m}(k),r_{j,i,m}(k)\right) 
    % \Sbarjimk = \Btwo\left(\bar{c}_{j,i,m}(k), \bar{r}_{j,i,m}(k)\right),
\end{equation}
% where each $S_{j,i,m}(q(\cdot;k))$ is an $L_2$ ball in $\mathbb{R}^3$ and $n_S \in \N$ is a user specified parameter.
where each $S_{j,i,m}(q_j(T_i; k))$ is an $L_2$ ball in $\mathbb{R}^3$, $n_S \in \N$ is a parameter that specifies the number of closed balls overapproximating each of the robot's links, and $k$ is a trajectory parameter that characterizes the motion of the robot over $T$.
\end{thm}
\noindent Note that one can explicitly construct an $\sfo$ that satisfies this assumption using the approach described in \cite{michaux2024sparrows}.
% For convenience, we summarize for convenience in Appendix \ref{app:reachability}.
% \noindent Note that one can explicitly construct an $\sfo$ that satisfies this assumption using the approach described in \cite{michaux2024sparrows}, which we summarize for convenience in Appendix \ref{app:reachability}.





==> sections/symbols.tex <==
\section*{List of Symbols}
\subsection*{Colors}
\begin{itemize}
    \item Red - obstacles
    \item Purple - reachable set
\end{itemize}

\subsection*{Generic Mathematical Symbols}
\begin{itemize}
%   \item $\lambda_j$: indeterminants
\item $\hat{e}_l$
  \item $n$: generic constant
  \item $\mathbb{N}$: natural numbers
  \item $\mathbb{R}^n$: reals 
%   \item $S_i(t)$: sliced reachable set
  \item $X$: a general set and/or metric space
\end{itemize}

\subsection*{Zonotope Symbols}
\begin{itemize}
    \item $Z$: generic zonotope
    \item $Z_1$: generic zonotope
    \item $Z_2$: generic zonotope
    \item $Z_1^g$: a zonotope with a center at the origin and the same generators of a zonotope, $Z_1$
    \item $Z_2^g$: a zonotope with a center at the origin and the same generators of a zonotope, $Z_2$
    \item $\beta_i$: zonotope indeterminants
    \item $\beta_{\forall}$: all indeterminants of a zonotope
    \item $c$: zonotope center
    \item $g_i$: ith zonotope generator
    \item $g_{\forall}$: all generators of a zonotope
    \item $\pzgi$: ith PZ coefficient (aka generator)
    \item $G_i$:  ith generator matrix of Matrix zonotope 
    \item $\nhj$: number of halfspaces of $\Pj$
    \item $M$: matrix zonotope
    \item $\pzn$: number of PZ generators
    \item $p_1$: generic point inside poly zonotope
    \item $p_2$: generic point inside poly zonotope
    %   \item $PZ$: generic polynomial zonotope
    \item $\pz{P_1}$: generic polynomial zonotope
    \item $\pz{P_2}$: generic polynomial zonotope
    \item $\Pj$: convexhull of $j$-th link's buffered FRS
    \item $\pz{R_{i-1}^i}$: poly zonotope representation of orientation of frame $i-1$ \textit{wrt} frame i
    \item $\pzv$: indeterminant for polynomial zonotope
    \item $\pzgi$: ith PZ coefficient (aka generator)
    \item $\sigma$: coefficient to be sliced/evaluated
\end{itemize}

\subsection*{SDF Symbols}
\begin{itemize}
  \item $\dist(\cdot)$: distance function
  \item \jon{need a symbol for sdf}
\end{itemize}

\subsection*{Coordinate frames and Transformations}
\begin{itemize}
    \item $p_i$: position of frame $i$ relative to frame $0$
    \item $p_{i-1,i}^i$: position of frame i wrt frame i-1 expressed in frame i \jon{i think this is not needed}
    \item $Q$: configuration space
    \item $R_{i-1}^i$: orientation of frame $i-1$ \textit{wrt} frame $i$
    \item $R_i(q)$: orientation of frame $i$ \textit{wrt} frame $0$
    \item $^Wx$: point $x$ represented in the world frame $W$
    \item $W$: world frame
    \item $W_s$ workspace frame of the robot
  \item $\omega_i^i$: frame i angular velocity wrt frame i
  \item $\dot{\omega}_i^i$: frame i angular acceleration wrt frame i
\end{itemize}

\subsection*{Trajectory Symbols}
\begin{itemize}
    \item $\kscale$: scale for $k$ interval
    \item $i$: time index
    \item $k$: trajectory parameter
    \item $K$: space of trajectory parameters
    \item $\nt$: number of time steps
    \item $j\in\Nq$: $j\in\{1,\cdots,\nq\}$
    \item $i\in\Nt$: $i\in\{1,\cdots,\nt\}$
    \item $h\in\Nhj$: $h\in\{1,\cdots,\nhj\}$
    \item $t$: time
    \item $t_i$: indexed time
    \item $T$: time interval
\end{itemize}

\subsection*{SJO Symbols}
\begin{itemize}
  \item $\pzCjiK$
  \item $\pzuj$
\end{itemize}

\subsection*{SLO Symbols}
\begin{itemize}
  \item 
\end{itemize}

\subsection*{SFO symbols}
\begin{itemize}
    \item 
    \item $c_{j,m}(k)$: The center of the m$^{th}$ sphere on the $j^{th}$ link
    \item $j$: index for specifying joint/link
    \item $\ell_{j,m}(k)$:
    \item $p_{j,1}$: Link $j$'s cap that is closer to the base in the kinematic tree. Also the center of joint $j$. 
    \item $p_{j,2}$: Link $j$'s cap that is closer to the ee in the kinematic tree. Also the center of joint $j+1$.
    \item $p_{j,2} = p_{j+1,1}$ \jon{correct?}
    \item \jon{Maybe we should just use $p_j(k)$ and $p_{j+1}(k)$}
    \item \jon{Should we label all the sphere centers with $c$? Right now the end caps have label $p$}
    \item $r_{j,m}(k)$: The radius of the m$^{th}$ sphere on the $j^{th}$ link
    \item $s(k)$: \jon{I think this symbol depends on the specific joint/link?}
    \item $s'(k)$: \jon{I think this symbol depends on the specific joint/link?}
    \item \adam{thinking about it after crappily writing the section, we should split the SFO to two parts - the Spherical Joint Occupancy, and the Spherical Link Occupancy. As such, we may want separate symbols for the joint center\&radii and the corresponding link ones. maybe a superscript $(l)$ or $(j)$, like $r^{l}_{j,m}$?}
    \item \adam{use $c$, $r$ for joints, $\bar{c}$, $\bar{r}$ for links, subscript tjm}
    
    \item $j$: index for specifying link
    \item $t$: index for specifying time interval
    \item $m \in \{1, 2\}$: index for specifying cap sphere of links, or the joint spheres in the Spherical Joint Occupancy. $1$ is closer to the base in the kinematic tree. $2$ is closer to the end effector in the kinematic tree.
    \item $i$: index for specifying the sphere on the link in the Spherical Link Occupancy
    \item $\mathbf{C}_{t,j,m}$: PZ for the center of joint sphere $m$ in the Joint Spherical Occupancy for link $j$ at the $t^{th}$ time interval.
    \item $c_{t,j,m}$: Some point center of joint sphere $m$ in the Joint Spherical Occupancy for link $j$ at the $t^{th}$ time interval, sliced from $\mathbf{C}_{t,j,m}$.
    \item $r_{t,j,m}$: Radius of the respective joint sphere.
    \item $S_{t,j,m} = (c_{t,j,m}, r_{t,j,m})$: Joint spheres for link $j$ at time interval $t$.
    \item $\mathbf{S}_{t,j,m} = (\mathbf{C}_{t,j,m}, r_{t,j,m})$: Spherical Joint Occupancy for joint $m$ related to link $j$ at time interval $t$.
    \item $S_{t,j,2} = S_{t,j+1,1}$ and $\mathbf{S}_{t,j,2} = \mathbf{S}_{t,j+1,1}$
    \item $\bar{c}_{t,j,\ell}(k)$: Center of the $i^{\text{th}}$ sphere on the $j^{\text{th}}$ link for the $t^{\text{th}}$ time interval in the Spherical Link Occupancy
    \item $\bar{r}_{t,j,\ell}(k)$: Radius of the $i^{\text{th}}$ sphere on the $j^{\text{th}}$ link for the $t^{\text{th}}$ time interval in the Spherical Link Occupancy
    \item $\bar{S}_{t,j,\ell} = (\bar{c}_{t,j,\ell}, \bar{r}_{t,j,\ell})$: Joint spheres for link $j$ at time interval $t$.
    \item \adam{$c$ is used for both the sphere centers and the centers of the joint spheres}
\end{itemize}



\newpage
